Examining Identity Drift in Conversations of LLM Agents

Large Language Models (LLMs) show impressive conversational abilities but sometimes show identity drift problems, where their interaction patterns or styles change over time. As the problem has not been thoroughly examined yet, this study examines identity consistency across nine LLMs. Specifically, we (1) investigate whether LLMs could maintain consistent patterns (or identity) and (2) analyze the effect of the model family, parameter sizes, and provided persona types. Our experiments involve multi-turn conversations on personal themes, analyzed in qualitative and quantitative ways. Experimental results indicate three findings. (1) Larger models experience greater identity drift. (2) Model differences exist, but their effect is not stronger than parameter sizes. (3) Assigning a persona may not help to maintain identity. We hope these three findings can help to improve persona stability in AI-driven dialogue systems, particularly in long-term conversations.

==> section/02_questions.tex <==
\section{Research Questions}
\label{sec:rq}

%In summary, this paper investigates the following research questions. This section details the hypotheses for each aspect of psychological states.
% In this study, we investigate the following research questions. 
This study investigates the following questions.
\begin{enumerate}[{RQ}1.]
    \item How does conversation depth affect the psychological states of LLMs?
    \item How do these psychological changes differ across various LLMs?
\end{enumerate}

Following PsychoBench \citep{psychobench}, we measure four aspects of an LLM's psychological states: \textit{personality}, \textit{interpersonal relationships}, \textit{motivation}, and \textit{emotion}. Appendix \ref{app:quest} elaborates questionnaires in each aspect. Here, we briefly name the questionnaires with hypotheses.

First, the personality aspect provides insights into the character, behavior, thoughts, and feelings of LLMs  \citep{psychobench}. While lifelong conversations influence human personality, a short conversation typically does not change human personality \citep{blonigen2008stability}. Thus, we expect personality measures to remain unchanged when LLMs accurately mimic human behaviors. To test this hypothesis, we focus on three questionnaires used in PsychoBench: the Big Five Inventory (BFI; \citet{BFI}), the revised version of the Eysenck Personality Questionnaire (EPQ-R; \citet{EPQ-R}), and the Dark Triad Dirty Dozen (DTDD, \citet{DTDD}) tests. We also anticipate that behaviors will differ across models as variations in pretraining data or parameter sizes lead LLMs to learn from different amounts of conversational data.

\begin{enumerate}[{H}1{-1}.]
    \item \textit{Personality remains unchanged.} 
    \item \textit{LLMs show different personality changes.} 
\end{enumerate}

Second, the interpersonal relationship aspect provides information about the internal dynamics of LLMs during social interactions \citep{psychobench}. PsychoBench used questionnaires to assess how LLMs generally perceive themselves and others without direct conversation. We used four questionnaires including Bem's Sex Role Inventory (BSRI; \citet{BSRI1, BSRI2}), Comprehensive Assessment of Basic Interests (CABIN; \citet{CABIN}), Interpersonal Competence Battery (ICB; \citet{ICB}), and a revised version of Experiences in Close Relationships (ECR-R; \citet{ECR-R1, ECR-R2}). However, such perceptions can change in the human mind during a social interaction \citep{aron1997experimental}. Thus, we assumed that interpersonal relationships will change as conversation depth increases for all LLMs. Additionally, deeper conversations can enhance intellectual intimacy, thereby improving mutual understanding \citep{laurenceau1998intimacy}. To capture such changes in mutual perception, we additionally use the McGill Friendship Questionnaire - Friend's Function  (MFQ-FF; \citet{McGill}), which directly assesses one's perception of conversation partners.

\begin{enumerate}[{H}1{-2}.]
    \item \textit{Interpersonal relationships increases.} 
    \item \textit{LLMs show similar trends in interpersonal relationships.} 
\end{enumerate}

Third, the motivation aspect provides insight into what triggers an individual's actions within specific contexts \citep{psychobench}. Like personality, a short conversation may not change one's motivation, while lifelong conversations can shape it. Therefore, like personality, we expect motivation to remain unchanged in a relatively short conversation. We also expect that different training setups may affect the motivation of LLMs.

\begin{enumerate}[{H}1{-3}.]
    \item \textit{Motivation remains unchanged.}
    \item \textit{LLMs show different motivational changes.}
\end{enumerate}

Finally, the emotional aspect assesses the ability to understand human emotions \citep{psychobench}. Following PsychoBench, we used three questionnaires: the Emotional Intelligence Scale (EIS; \citet{EIS}), Wong and Law Emotional Intelligence Scale (WLEIS; \citet{WLEIS}), and Empathy Scale (Empathy; \citet{empathy}). As with personality and motivation, a short conversation is unlikely to influence the emotional aspect since these questionnaires measure emotional ability. Therefore, we expect the emotional aspect to remain constant as conversations deepen. Additionally, emotional abilities may differ depending on the specific LLM used.

\begin{enumerate}[{H}1{-4}.]
    \item \textit{Emotion remains unchanged.}
    \item \textit{LLMs show different emotional changes.}
\end{enumerate}




% \section{Research Questions}
% \label{sec:rq}

% In summary, this paper investigates the following research questions. This section describes detailed hypotheses for each aspect of psychological states.
% \begin{enumerate}[{RQ}1.]
%     \item How does conversation depth change the psychological states of LLMs?
%     \item How such psychological changes are different across different LLMs?
% \end{enumerate}

% Following \citet{psychobench}, we measure four aspects of LLM's psychological states: \textit{Personality}, \textit{Interpersonal Relationships}, \textit{Motivation}, and \textit{Emotion}. First, the personality aspect provides information about LLM's character, behavior, thoughts, and feelings \citep{psychobench}. Though the personality of a human being is affected by life-long conversations, a short conversation seldom changes one's personality \citep{blonigen2008stability}. Thus, when LLMs mimic human behaviors correctly, we expect that personality measures should be unchanged. To test such a hypothesis, we focus on three questionnaires as in PsychoBench: Big Five Inventory (BFI; \citet{BFI}), the revised version of the Eysenck Personality Questionnaire (EPQ-R; \citet{EPQ-R}), and Dark Triad Dirty Dozen (DTDD, \citet{DTDD}) tests. Also, we expect the behavior to differ across models since pretraining data or parameter sizes make LLMs learn different amounts of conversations.

% \begin{enumerate}[{H}1{-1}.]
%     \item \textit{Personality will remain unchanged.} 
%     \item \textit{LLMs show different Personality behavior.} 
% \end{enumerate}

% Second, the interpersonal relationship aspect provides information about LLM's internal dynamics of social interactions \citep{psychobench}. In PsychoBench, they used questionnaires about how LLMs generally perceive themselves and others without having a conversation. The four questionnaires include Bem's Sex Role Inventory (BSRI; \citet{BSRI1, BSRI2}), Comprehensive Assessment of Basic Interests (CABIN; \citet{CABIN}), Interpersonal Competence Battery (ICB; \citet{ICB}), and a revised version of Experiences in Close Relationships (ECR-R; \citet{ECR-R1, ECR-R2}). However, in a human mind, such perceptions can be changed during a social interaction \citep{aron1997experimental}. Therefore, we expect that interpersonal relationships will change as conversation depth becomes deeper for any LLMs. Also, the depth of conversation can strengthen intellectual intimacy, thereby improving mutual understanding \citep{laurenceau1998intimacy}. To capture such changes in mutual perception, we additionally used the McGill Friendship Questionnaire (MFQ; \citet{McGill}), which directly questions one's perception of conversation partners.

% \begin{enumerate}[{H}1{-2}.]
%     \item \textit{Interpersonal Relationship increases.} 
%     \item \textit{LLMs show similar trends on Relationship.} 
% \end{enumerate}

% Third, the motivation aspect provides information about the trigger of one's action within specific contexts \citep{psychobench}. Similar to personality, a short conversation may not change one's motivation in the human mind, though life-long conversation can help form one's motivation. Therefore, similar to the personality aspect, we expect the motivation will remain unchanged as a conversation goes deeper. We also expect that different training setups can change the behavior of motivational aspects across LLMs.

% \begin{enumerate}[{H}1{-3}.]
%     \item \textit{Motivation will remain unchanged.}
%     \item \textit{LLMs show different Motivation behavior.}
% \end{enumerate}

% Lastly, the emotional aspect provides information about the ability to understand human emotions \citep{psychobench}. Following PsychoBench, we used three questionnaires: Emotional Intelligence Scale (EIS; \citet{EIS}), Wong and Law Emotional Intelligence Scale (WLEIS; \citet{WLEIS}), and Empathy Scale (Empathy; \citet{empathy}). Similar to Personality or Motivation, a short conversation may not change the emotional aspect since these three measure emotional ability. Thus, we expect the emotional aspect to remain the same when a conversation becomes deeper. Also, such emotional ability will behave differently when we use different LLMs.

% \begin{enumerate}[{H}1{-4}.]
%     \item \textit{Emotion will remain unchanged.}
%     \item \textit{LLMs show different Emotion behavior.}
% \end{enumerate}


% \quad\textbf{RQ1}. \textit{How do multi-agent interactions influence changes in LLMs' psychological trait?} %, and to what extent does parameter size contribute to these changes?}

% As the depth of the conversation increases, changes are expected to occur in the domain of Interpersonal Relationships. This hypothesis is based on findings from human studies, which indicate that deeper conversations lead to enhanced Emotional and Intellectual Intimacy \citep{collins1994self, aron1997experimental}. In human interactions, the depth of conversation strengthens emotional and intellectual intimacy, thereby improving mutual understanding and empathy \citep{laurenceau1998intimacy}. Therefore, if LLMs mimic human interactions, it is likely that similar patterns will be observed in LLM interactions as well. On the other hand, fixed and intrinsic psychological factors such as Personality Traits, Emotional Abilities, and Motivational Test are not expected to change significantly during short-term interactions. This expectation is grounded in psychological theories suggesting that human personality and emotional abilities are shaped by long-term experiences and learning \citep{blonigen2008stability}. 

%Multi-agent interactions are expected to be a key factor influencing changes in LLMs' social intelligence. Drawing from human studies, deeper conversations tend to enhance emotional and intellectual intimacy, leading to better mutual understanding and empathy between individuals \citep{collins1994self, aron1997experimental}. Similarly, in the case of LLMs, as the depth and quality of conversations increase, it is hypothesized that notable changes will occur in the domain of interpersonal relationships. This may manifest in improved social understanding and communication skills, as LLMs emulate human conversational dynamics. Therefore, the depth and nature of multi-agent conversations are expected to play a critical role in driving these changes.

%In addition to conversational depth, model parameter size is another factor that could potentially affect the changes in social intelligence during multi-agent interactions. Previous research suggests that larger models tend to perform better in tasks requiring logical reasoning and problem-solving abilities \citep{parametergood}. However, social intelligence is a multifaceted ability that encompasses emotional understanding, interpersonal relationships, and empathy, areas that may not rely solely on logical reasoning or the computational capacity provided by larger models. It remains unclear to what extent parameter size directly contributes to these abilities, as they are also shaped by the quality of interaction experiences and the data on which the models have been trained.

%대화가 깊어짐에 따라 Interpersonal Relationship 영역에서 변화가 나타날 것으로 예상된다. 이는 인간 연구에서 깊이 있는 대화가 이루어질수록 Emotional Intimacy, Intellectual Intimacy이 향상된다는 연구 결과를 바탕으로 한 가설이다 \citep{collins1994self,aron1997experimental}. 인간 상호작용에서 대화의 깊이는 감정적 및 지적 Intimacy를 강화하며, 이를 통해 상호간의 이해와 공감 능력이 증진된다 \citep{laurenceau1998intimacy}. 따라서 LLM이 인간의 상호작용을 mimic한다면, LLM 간의 상호작용에서도 이러한 패턴이 반복될 가능성이 높다. 반면, Personality Traits Emotional Abilities, Motivational Test와 같은 고정적이고 본질적인 심리적 요소는 단기간의 상호작용으로는 크게 변화하지 않을 것으로 예상된다. 이는 인간의 성격 및 감정 능력이 장기적 경험과 학습에 의해 변화한다는 심리학 이론에 기반하고 있다 \citep{blonigen2008stability}.


%\quad\textbf{RQ2}. \textit{Can parameter size affect LLMs' social intelligence during the conversation?}

%There is a known correlation between the parameter size of an LLM and its performance, with prior studies reporting that larger parameter sizes lead to improvements in logical reasoning and problem-solving abilities \citep{parametergood}. However, complex abilities such as Social Intelligence, which do not heavily rely on logical reasoning, are less likely to be influenced solely by the size or computational capacity of the model. Social Intelligence encompasses various factors, including Emotional and Interpersonal Relationships, and the performance of the model is significantly affected not only by its parameter size but also by the data it has been trained on. In our experiment, the quality of conversations and interaction experiences may have a greater impact on the results. Therefore, we anticipate that the effect of parameter size on changes in Social Intelligence observed during interactions will be limited in our study.
%LLM의 Parameter size와 성능 간에는 일정한 상관관계가 존재하며, 특히 논리적 추론과 문제 해결 능력은 파라미터 크기가 클수록 향상된다는 선행 연구들이 보고된 바 있다 \citep{parametergood}. 그러나 Social Intelligence와 같이 다면적이지만 논리적 추론이 크게 필요하지 않은 능력은 단순히 모델의 크기나 처리 능력에 의해 좌우되지 않을 가능성이 높다. %Social Intelligence는 Emotional, Interpersonal Relationship등 다양한 요소를 포함하며, 또한, 모델의 성능에는 parameter size 뿐만 아니라 학습한 데이터가 크게 영향을 미치므로, 우리 실험의 경우 대화의 질이나 상호작용 경험에 더 큰 영향을 받을 수 있다. 따라서 우리의 연구에서는 Parameter Size가 대화 중 나타나는 Social Intelligence 변화에 미치는 영향이 제한적일 것으로 예상한다. 



%
%\paragraph{Study 2.}  Study 1에서 특정 질문지 형식을 따르는 한계로 인해 일반화가 어려운 점을 보완하기 위해, Study 2에서는 일상 대화로 구성된 기존의 대화 시스템 데이터셋을 활용하여 LLM 간 상호작용을 유도하고, 각 단계마다 LLM의 특성 변화를 분석하였다. 일반화 가능성을 높이기 위해, 일상 대화뿐만 아니라 다양한 상황을 포함하도록 주제를 설정하고(Topic), 다양한 감정 상태를 반영하여(Emotion) Social Intelligence의 변화를 두 가지 측면에서 평가하였다.\citep{taskmaster,dailydialog}.


% 감정 데이터셋, 대화 데이터셋

%\quad\textbf{RQ3}. \textit{Can conversation between multi-agents change LLMs' social intelligence?}

%LLM 간의 상호작용이 다양한 상황에서 대화가 깊어질수록 Social Intelligence에 미치는 영향을 분석할 때, LLM이 프롬프트에 민감하게 반응하는 특성을 고려해야 한다\citep{}. LLM은 prompt의 구조와 맥락에 따라 민감한 반응을 보이며, 이는 감정적 이해 및 대화의 맥락 이해와 관련된 성능에 영향을 미친다 \citep{}. 

%\textbf{Topic} 일상 대화에서 주제를 중심으로 LLM 간 반복적 상호작용을 유도하면 Interpersonal Relationship 능력이 향상될 가능성이 높다. 이는 Study 1의 RQ1에서 제시된 가설과 일치하며, 일상 대화에서의 자연스러운 상호작용이 대인 관계 형성 능력에 긍정적인 영향을 미칠 수 있음을 시사한다. 또한, 주제에 맞는 대화를 통해 LLM이 맥락과 대화의 흐름을 더 잘 이해하게 되어, 대화의 목표에 맞는 반응을 학습함으로써 Motivational Test의 일부 항목에서도 성능 향상이 나타날 수 있다. 그러나 이러한 향상은 프롬프트의 민감성과 대화의 질에 크게 좌우될 것으로 예상된다 \citep{}.

%\textbf{Emotion} 감정적 대화 상황에서는 LLM이 상호작용 중 생성한 감정적 발화의 영향을 받아 Emotional Abilities가 향상될 것으로 예상된다. 감정적으로 풍부한 대화를 통해 LLM은 감정 인식 및 표현 능력을 강화하고, 다양한 감정 상태에 적절하게 대응하는 능력을 발전시킬 수 있다. 그러나 Personality Traits는 강렬한 감정적 대화에서 약간의 변화를 보일 수 있지만, 전반적으로는 큰 변화를 보이지 않을 것으로 예상된다 \citep{blonigen2008stability}.

%따라서, 두 가지 상황에서 LLM의 Social Intelligence 변화는 상호작용의 맥락과 프롬프트에 대한 민감성에 따라 상이하게 나타날 수 있다.

%\quad\textbf{RQ4}. \textit{Can parameter size affect LLMs' social intelligence during the conversation?}

%LLM의 Parameter 크기가 Social Intelligence에 미치는 영향을 분석할 때, 파라미터 크기가 큰 모델은 논리적 추론과 문제 해결 능력에서 우수한 성능을 발휘하지만 \citep{}, 프롬프트에 대한 민감성으로 인해 Social Intelligence와 같은 영역에서는 모델 크기보다는 학습된 데이터의 질과 다양성이 더 중요한 요소로 작용할 가능성이 높다 \citep{}.

%\textbf{Topic} 일상 대화와 특정 주제를 중심으로 한 상호작용에서는 모델의 자연스러운 대화 능력이 Social Intelligence에 큰 영향을 미칠 것으로 예상된다. 만약 특정 주제에 대해 자연스럽고 유연한 대화가 불가능할 경우, 대화의 깊이가 깊어질수록 대화의 일관성 및 대인관계 형성 능력 등 전반적인 영역에서 성능 저하가 발생할 것으로 예상한다. 따라서, 대화의 깊이에 따른 Social Intelligence 변화 폭이 HellaSwag 벤치마크의 점수와 밀접하게 연관될 것으로 보이며, 높은 논리적 일관성을 보이는 모델일수록 대화 주제에 따른 Social Intelligence의 변화 폭이 증가할 가능성이 크다.

%\textbf{Emotion}
%감정적 상황을 중심으로 한 상호작용에서는 모델의 학습 데이터가 큰 영향을 미칠 것으로 예상된다. 만약 LLM이 감정적 발화를 효과적으로 생성할 수 있다면, 대화가 심화될수록 프롬프트의 영향으로 인해 Emotional Abilities 점수가 증가할 수 있다. 그러나 감정 표현 능력 외의 다른 영역에서는 변화가 미미할 것으로 보인다. 이는 감정적 대화 상황에서 Interpersonal Relationship이나 Motivational Test와 같은 영역보다는 Emotional Abilities가 더 크게 영향을 받을 가능성이 높기 때문이다.

%따라서, LLM의 Social Intelligence 변화에 있어 파라미터 크기보다는 학습된 데이터의 질과 특성이 더 중요한 영향을 미칠 것으로 예상된다. Social Intelligence의 변화는 학습 데이터가 다루는 주제와 감정 상황의 다양성 및 질에 크게 의존하며, 이는 모델의 성능 차이보다는 데이터의 특성에 의해 결정될 가능성이 높다.


% H3. 인간의 심리학 실험 디자인에서 생성된 결과와 Dialogue dataset을 기반의 데이터로 얻은 결과의 변화 양상 추이는 비례할 것이다.

%첫째, LLM-LLM 상호작용을 통한 태스크 해결에만 관심을 두었을 뿐, LLM에게 부여된 prompt 특성이 상호작용 동안 얼마나 일관되게 유지되는지에 대한 연구가 부족하다. 이는 LLM이 다양한 상황에서 prompt에 따라 일관된 행동을 보일 수 있는지, 아니면 상호작용을 통해 변화하는지를 이해하는 데 중요한 요소이다.

% [문단] 한계2: Mimic이 제대로 되는지 확인하는 과정이 없거나 약하다
%둘째, Human의 Behavior을 mimic 할 수 있는지 확인하는 과정이 충분히 이루어지지 않았거나 약한 경우가 많다. LLM에게 인간 심리학 테스트를 적용하여 LLM이 Human의 Behavior을 모방할 수 있는지를 연구하는 시도가 활발하게 이루어지고 있지만, 대부분의 연구는 단일 LLM에서만 이러한 행동 모방을 확인했다. LLM 간 상호작용에서의 심리학적 특성을 확인한 연구는 매우 드물며, 우리가 아는 한, LLM-LLM 상호작용을 다룬 연구는 \citet{llminteraction1}이 유일하다. \citet{llminteraction1}에서는 LLM의 성격 특성 변화를 관찰했지만, 이는 GPT 시리즈 모델에만 한정되어 있었고, 더 다양한 모델과 상호작용을 다루지 못했다는 한계가 있다.

% 이렇게 적으면 인간 결과를 보여주교 비교하는 방향으로 연구를 잡아야함.
% Interaction을 사람과 비교하는 것을 확인해야한다라는 방향으로 움직이는 것이 아니라, LLM한테 일어나는 Interaction 변화를 확인해야한다라는 느낌으로 서술해야할듯

%종합해보면, LLM-LLM의 Interaction이 진행됨에 따라 Human의 심리적 특성과 유사하게 변화하는지를 확인할 필요가 있지만, 이 부분에 대한 연구는 아직 충분히 이루어지지 않았다. 심리학 분야에서는 인간의 Social Intelligence가 친밀감과 깊은 연관이 있다는 사실이 잘 알려져 있다. 연구에 따르면, 인간은 Interaction을 거듭할수록 친밀감이 증가하며, 이와 함께 사회적 지능과 친밀감 간의 밀접한 상관관계도 보고된 바 있다. 따라서 LLM 간의 상호작용이 인간의 이러한 특성을 얼마나 모방할 수 있는지를 연구하는 것이 필요하다.

%이러한 점을 종합해보면, LLM-LLM의 상호작용이 깊어지면서 LLM-LLM간의 상호작용이 실제 인간의 심리학적 특성과 유사하게 변화하는지 확인할 필요가 있지만, 아직 깊게 연구되지 않았다.

% [문단] 가설 및 실험에 대한 소개
% 따라서, 우리는 LLM - LLM간의 상호작용이 깊어질수록 인간의 심리학적 특성과 유사하게 변화하는지 확인하기 위해 인간에게 수행한 심리학 실험을 LLM에게 적용하고자한다. 

%따라서, 우리는 LLM간의 상호작용이 깊어질수록 인간과 유사한 행동 패턴이 나타나는지 확인하고 분석하고자한다.
% 우선 심리학에서 사용한 질문지를 활용 -> Psychobench + PAIR test 적용하고, -> 실제 AI System에서도 영향을 미치는지 확인하기 위해 Dialog Dataset을 활용해 동일한 실험을 진행하여 비교하고, 실제로 Score에 영향을 미치는지까지 확인한다.

%따라서, 우리는 LLM - LLM Interaction에 따른 변화가 Human이랑 유사한지 확인한다.우선, 심리학적 실험을 활용하여 LLM 간의 상호작용이 깊어질수록 LLM의 친밀감과 사회적 지능이 증가하는지를 확인하고 언어모델의 상호작용에 특화된 Dialog Dataset을 활용하여 Conversation간 LLM이 친밀감과 사회적 지능이 증가하는 확인하여, 이러한 변화가 친밀감과 LLM의 상호작용 성능에 미치는 영향을 확인한다. 

%우리는 LLM이 언어에 기반한 모델이라는 점을 고려하여, 언어를 활용한 대표적 상호작용인 대화를 활용한다. 대화를 통한 상호작용이 깊어질수록 LLM 간 친밀감과 Social Intellegece가 증가하는지를 확인하고자 한다. 먼저, 통상적으로 자주 쓰이는 LLM에 대한 분석을 통해 LLM의 전반적인 경향을 확인한다.  1) 모델의 파라미터 크기에 따른 변화를 비교한다.

%우리는 LLM의 사회적 지능을 확인하기 위해 기존 심리학 실험을 기반으로 만들어진 벤치마크인 PsychoBench를 활용한다. 추가적으로 LLM 간의 상호작용 간 친밀감 변화를 확인하기 위해, 인간의 상호작용에 따른 친밀감을 측정할 수 있는 심리학 설문지를 활용한다. 더하여, LLM 간의 상호작용을 위하여 대화가 진행될수록 서로 간의 상호작용이 깊어지는 질문지를 활용한다.

%우리의 가설은 다음과 같다.
%H0. 모든 모델에서 대화 이전보다 대화 이후에 친밀감 형성이 이뤄질 것이다.
%H0-1. 대화가 깊어질수록 Emotional Intimacy, Intellectual Intimacy, Conventionality가 증진될 것이다.

%- 해당 영역은 대화에서 공통되는 부분이 상대적으로 적어도 대화가 매끄럽게 진행되는 영역들이다. 그러므로 Context길이가 길어지더라도, 본인의 자세한 Persona의 간섭을 덜 받을 것으로 예상하기 때문에 대화가 깊어질수록 이 영역의 PAIR 점수가 증가할 것으로 예상한다.

%H0-2. 대화가 깊어지는 것과 Social Intimacy, Recreational Intimacy는 연관성이 없을 것이다.

%- 해당 영역은 대화에서 공통되는 부분이 많아야지 높은 친밀감을 느끼는 영역이다. 하지만 Context길이가 길어질수록 LLM이 과거의 내용을 정확하게 기억하지 못하는 문제로 인하여 할루시네이션이 일어나서 대화가 매끄럽게 진행되지 않을 것으로 예상한다. 그러므로, 대화가 깊어지더라도 PAIR 점수가 높게 생성되지 않을 것으로 예상한다.

%H0-3. 대화가 깊어지더라도 Sexual Intimacy에는 변화가 없을 것이다.

%- LLM의 Ethical Policy로 인해 생성되는 텍스트가 조절되기 때문에, 성적 지향과 관련된 문항들에는 반응하지 않으려 할 가능성이 높다.


%H1. 모델 크기와 무관하게 친밀한 관계 형성 정도에 차이가 없을 것이다.

%H1-1. 모델 크기에 따른 친밀감 형성 정도(stage3 PAIR - stage0 PAIR)에 차이가 없을 것이다. // 

%- 모델 사이즈는 LLM이 학습한 양에 비례한다. 데이터의 양이 많다고 해서, 친밀한 관계 형성 정도에는 차이가 없을 것으로 예상한다.

%H2. PsychoBench의 결과는 일부 영역은 오르지만, 일부 영역은 변화가 없을 것이다.

%H2-1 대화가 깊어질수록 Emotional Ability와 Interpersonal Relationships 점수가 상승할 것이다.
%인간은 깊이있는 대화가 이어질수록 공감능력과 대화능력이 상승하기 때문에 LLM도 그에 따라 공감능력과 대하능력이 상승할 것으로 예상된다.

%H2-2 대화가 깊어질수록 Personality trait과 Motivational test 점수는 변화가 없을 것이다.
%인간은 깊이있는 대화가 이어질수록 공감능력과 대화능력이 상승하지만 성격과 동기에 관한 영역은 큰 변화가 없다. 그러므로, LLM도 마찬가지로 Personality trait과 Motivational Test점수는 변화가 없을 것이다..


%H3. Emotional Ability와 Interpersonal Relation ships 점수와 PAIR test 점수는 비례해서 상승할 것이다.

%- Human의 경우 친밀감과 Social Intelligence는 비례하는 경향이 있다. 특히, 친밀감과 가장 연관된 Social Intelligence는 Emotional Ability와 Interpersonal Relation ship이다. 그러므로 Social Intelligence와 Emotional Ability는 비례해서 증가하게 될것이다.

%H4. 인간의 실제 심리학 실험을 LLM에 적용하였을 때의 점수 변화와, 이에 비례하는 Dialog Dataset Score의 변화는 비례할 것이다.
% Dailydialog >> 대인관계
% EmpatheticDialogues >> 감정
% [성격 >] ConvAI2 >> 친밀감


==> table/01_personality_old.tex <==
\renewcommand{\arraystretch}{0}
\begin{table*}
    \centering
    \begin{tabular}{lr|cc|cccc|cc|cc}
    
    \toprule
     & {\small \textit{Factors}} & \multicolumn{2}{c|}{GPT} & \multicolumn{2}{c}{LLaMA 3} & \multicolumn{2}{c|}{LLaMA 3.1} & \multicolumn{2}{c|}{Mixtral 8x} &
         \multicolumn{2}{c}{Qwen 2} \\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
    & & 3.5T & 4o & 8B & 70B & 70B & 405B & 7B & 22B & 7B & 72B \\
    \midrule
    
    \multicolumn{12}{@{}l}{\large \textbf{(1) Personality}}\\
    \midrule
    BFI & {\small \textit{Openness}} & \goinguppp & \goingdown & \goingstay & \goingrand & \goingstay & \goingdown & \goingstay & \goingstay & \goingstay & \goinguppp \\
     & {\small \textit{Conscientiousness}} & \goinguppp & \goingdown & \goingstay & \goingrand & \goingstay & \goingdown & \goingstay & \goingstay & \goingstay & \goingstay \\
     & {\small \textit{Extraversion}} & \goingrand & \goingdown & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingstay & \goingstay \\
     & {\small \textit{Agreeableness}} & \goinguppp & \goingdown & \goingstay & \goingrand & \goingstay & \goingdown & \goingstay & \goingstay & \goingstay & \goingstay \\
     & {\small \textit{Neuroticism}} & \goinguppp & \goingdown & \goingstay & \goingrand & \goingstay & \goingdown & \goingstay & \goingdown & \goingstay & \goingstay \\
    \midrule
    EPQ-R & {\small \textit{Extraversion}} & \goinguppp & \goingdown & \goingstay & \goingdown & \goingdown & \goingdown & \goingdown & \goingstay & \goingstay & \goingstay \\
     & {\small \textit{Psychoticism}} & \goinguppp & \goingdown & \goingstay & \goingdown & \goingdown & \goingdown & \goingdown & \goingstay & \goingstay & \goingstay \\
     & {\small \textit{Neuroticism}} & \goinguppp & \goingdown & \goingstay & \goingdown & \goingdown & \goingdown & \goingdown & \goingstay & \goingstay & \goingstay \\
     & {\small \textit{Lying}} & \goinguppp & \goingdown & \goingstay & \goingdown & \goingdown & \goingdown & \goingdown & \goingstay & \goingstay & \goingstay \\
    \midrule
    DTDD & {\small \textit{Machiavellianism}} & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goinguppp & \goingstay \\
     & {\small \textit{Psychopathy}} & \goingdown & \goingdown & \goingstay & \goingdown & \goingdown & \goingdown & \goingstay & \goingdown & \goingstay & \goingstay \\
     & {\small \textit{Narcissism}} & \goingdown & \goingrand & \goingstay & \goingdown & \goingdown & \goingdown & \goingstay & \goingdown & \goingstay & \goingstay \\
    \bottomrule
    \multicolumn{12}{c}{\phantom{M}}\\
    \multicolumn{12}{c}{\phantom{M}}\\
    \multicolumn{12}{@{}l}{\large \textbf{(2) Interpersonal Relationship}}\\
    \toprule
    BSRI & {\small \textit{Masculine}} & \goinguppp & \goingstay & \goinguppp & \goingrand & \goingdown & \goingdown & \goingstay & \goingdown & \goingstay & \goingstay \\
     & {\small \textit{Feminine}} & \goinguppp & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingstay & \goinguppp \\
    \midrule
    CABIN & {\small \textit{Realistic}} &  \goingstay & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
     & {\small \textit{Investigate}} & \goingstay & \goingrand & \goingdown & \goingstay & \goingdown & \goingstay & \goingstay & \goingstay & \goingdown & \goingdown \\
     & {\small \textit{Artistic}} & \goinguppp & \goingstay & \goingstay & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
     & {\small \textit{Social}} & \goingstay & \goinguppp & \goingdown & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
     & {\small \textit{Enterprising}} & \goingstay & \goingstay & \goingdown & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
     & {\small \textit{Conventional}} & \goingstay & \goingrand & \goingdown & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
    \midrule
    ICB & {\small \textit{Overall}} & \goingdown & \goingstay & \goingstay & \goingstay & \goinguppp & \goingstay & \goingstay & \goingstay & \goingstay & \goinguppp \\
    \midrule
    ECR-R & {\small \textit{Attachment Anxiety}} & \goingstay & \goingdown & \goingstay & \goingrand & \goingdown & \goingdown & \goingdown & \goingdown & \goinguppp & \goingstay \\
     & {\small \textit{Attachment Avoidance}} & \goinguppp & \goingdown & \goingstay & \goingrand & \goingdown & \goingdown & \goingstay & \goingstay & \goingrand & \goingstay \\
     \midrule
    MFQ & {\small \textit{Stimulating companionship}} & \goingdown & \goinguppp & \goingdown & \goingrand & \goinguppp & \goinguppp & \goingstay & \goinguppp & \goingstay & \goinguppp \\
     & {\small \textit{Help}} & \goingdown & \goinguppp & \goingdown & \goingrand & \goinguppp & \goinguppp & \goingstay &  \goinguppp & \goingstay & \goinguppp \\
     & {\small \textit{Intimacy}} & \goingdown & \goinguppp & \goingdown & \goingrand & \goinguppp & \goinguppp & \goingstay & \goinguppp & \goingstay & \goinguppp \\
     & {\small \textit{Reliable alliance}} & \goingdown & \goinguppp & \goingdown & \goingrand & \goinguppp & \goinguppp & \goingstay & \goinguppp  & \goingstay & \goinguppp \\
     & {\small \textit{Self-validation}} & \goingdown & \goinguppp & \goingdown & \goingrand & \goinguppp & \goinguppp & \goingstay & \goinguppp & \goingstay & \goinguppp \\
     & {\small \textit{Emotional security}} & \goingdown & \goinguppp & \goingdown & \goingrand & \goinguppp & \goinguppp & \goingstay & \goinguppp & \goinguppp & \goinguppp \\
    \bottomrule %Mixtral 시리즈만 추가 안함
    \multicolumn{12}{c}{\phantom{M}}\\
    \multicolumn{12}{c}{\phantom{M}}\\
    \multicolumn{12}{@{}l}{\large \textbf{(3) Motivation}}\\
    \toprule
        GSE & {\small \textit{Overall}} & \goingstay & \goingstay & \goinguppp & \goingrand & \goingrand & \goingstay & \goingrand & \goingstay & \goingrand & \goingdown \\
    \midrule
    LOT-R & {\small \textit{Overall}} & \goingrand & \goingrand & \goinguppp & \goingrand & \goinguppp & \goingstay & \goingstay & \goingstay & \goinguppp & \goinguppp \\
    \midrule
    LMS & {\small \textit{Rich}} & \goinguppp & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingrand & \goingstay \\
     & {\small \textit{Motivator}} & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goinguppp \\
     & {\small \textit{Important}} & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingrand & \goingstay \\
    \bottomrule
    \multicolumn{12}{c}{\phantom{M}}\\
    \multicolumn{12}{c}{\phantom{M}}\\
    \multicolumn{12}{@{}l}{\large\textbf{(4) Emotion}}\\
    \toprule
        EIS & {\small \textit{Overall}} & \goingrand & \goingdown & \goingstay & \goingrand & \goingdown & \goingdown & \goingstay & \goingdown & \goingdown & \goingdown \\
    \midrule
    WLEIS & {\small \textit{Self-emotion appraisal}} & \goingrand & \goingdown & \goinguppp & \goingdown & \goingstay & \goinguppp & \goingstay & \goinguppp & \goingdown & \goingrand \\
     & {\small \textit{Others' emotion appraisal}} & \goingrand & \goingdown & \goinguppp & \goingrand & \goingstay & \goinguppp & \goinguppp & \goinguppp & \goingdown & \goingrand \\
     & {\small \textit{Use of emotion}} & \goingrand & \goingdown & \goinguppp & \goingrand & \goingdown & \goinguppp & \goinguppp & \goinguppp & \goinguppp & \goingrand \\
     & {\small \textit{Regulation of emotion}} & \goingrand & \goingdown & \goinguppp & \goingrand & \goingdown & \goingstay & \goingstay & \goinguppp & \goingrand & \goingrand \\
    \midrule
    Empathy & {\small \textit{Overall}} & \goingrand & \goingdown & \goinguppp & \goingdown & \goingdown & \goingstay & \goingdown & \goingstay & \goingstay & \goingrand \\
    
    \bottomrule
    \phantom{M} \\
    \multicolumn{12}{r}{\small \goingstay\ Statistically Insignificant change, \goinguppp\ Consistently increased, \goingdown\ Consistently decreased, \goingrand\ Inconsistent change}
    \end{tabular}
    
    \caption{LLM's change in psychological states. We check the consistency with the sign of all $\Delta_{i, j}$ values ($i < j$). Detailed statistical results are shown in Appendix (Tables \ref{tab:app-full-1} and \ref{tab:app-full-3}).}
    \label{tab:result}
\end{table*}

==> table/02_interpersonal.tex <==
% \begin{table*}
%     \centering
%     \begin{tabular}{lr|cccccccccc}
%     \toprule
%      & {\small \textit{Factors}} & \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{LLaMA 3} & \multicolumn{2}{c}{LLaMA 3.1} & \multicolumn{2}{c}{Mixtral 8x} &
%          \multicolumn{2}{c}{Qwen2} \\
%     \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
%     \hspace{8ex}\phantom{.}&\hspace{19ex}\phantom{.}& 3.5T & 4o & 8B & 70B & 70B & 405B & 7B & 22B & 7B & 72B \\
%     \midrule
%     BSRI & {\small \textit{Masculine}} & \goinguppp & \goingstay & \goinguppp & \goingrand & \goingdown & \goingdown & \goingstay & \goingdown & \goingstay & \goingstay \\
%      & {\small \textit{Feminine}} & \goinguppp & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingstay & \goinguppp \\
%     \midrule
%     CABIN & {\small \textit{Realistic}} & \goingstay & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
%      & {\small \textit{Investigate}} & \goingstay & \goingrand & \goingdown & \goingstay & \goingdown & \goingstay & \goingstay & \goingstay & \goingdown & \goingdown \\
%      & {\small \textit{Artistic}} & \goinguppp & \goingstay & \goingstay & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
%      & {\small \textit{Social}} & \goingstay & \goinguppp & \goingdown & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
%      & {\small \textit{Enterprising}} & \goingstay & \goingstay & \goingdown & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
%      & {\small \textit{Conventional}} & \goingstay & \goingrand & \goingdown & \goingstay & \goingdown & \goingdown & \goingstay & \goingstay & \goingdown & \goingdown \\
%     \midrule
%     ICB & {\small \textit{Overall}} & \goingdown & \goingstay & \goingstay & \goingstay & \goinguppp & \goingstay & \goingstay & \goingstay & \goingstay & \goinguppp \\
%     \midrule
%     ECR-R & {\small \textit{Attachment Anxiety}} & \goingstay & \goingdown & \goingstay & \goingrand & \goingdown & \goingdown & \goingdown & \goingdown & \goingrand & \goingstay \\
%      & {\small \textit{Attachment Avoidance}} & \goinguppp & \goingdown & \goingstay & \goingrand & \goingdown & \goingdown & \goingstay & \goingstay & \goingrand & \goingstay \\
%      \midrule
%     MFQ & {\small \textit{Stimulating companionship}} & \goingstay & \goinguppp & \goingdown & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay \\
%      & {\small \textit{Help}} & \goingstay & \goinguppp & \goingdown & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay \\
%      & {\small \textit{Intimacy}} & \goingstay & \goinguppp & \goingdown & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay \\
%      & {\small \textit{Reliable alliance}} & \goingstay & \goinguppp & \goingdown & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay \\
%      & {\small \textit{Self-validation}} & \goingstay & \goinguppp & \goingdown & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay \\
%      & {\small \textit{Emotional security}} & \goingstay & \goinguppp & \goingdown & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay \\
%     \bottomrule
%     \multicolumn{12}{r}{\small \goinguppp Consistently increased, \goingdown Consistently decreased, \goingstay Insignificant change, \goingrand Inconsistent change}
%     \end{tabular}
    
%     \caption{LLM's change on Interpersonal Relationship ability over conversation}
%     \label{tab:interpersonal}
% \end{table*}

==> table/03_motivation.tex <==
% \begin{table*}
%     \centering
%     \begin{tabular}{lr|cccccccccc}
%     \toprule
%      & {\small \textit{Factors}} & \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{LLaMA 3} & \multicolumn{2}{c}{LLaMA 3.1} & \multicolumn{2}{c}{Mixtral 8x} &
%          \multicolumn{2}{c}{Qwen2} \\
%     \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
%     \hspace{8ex}\phantom{.}&\hspace{19ex}\phantom{.}& 3.5T & 4o & 8B & 70B & 70B & 405B & 7B & 22B & 7B & 72B \\
%     \midrule
%     GSE & {\small \textit{Overall}} & \goingstay & \goingstay & \goinguppp & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay \\
%     \midrule
%     LOT-R & {\small \textit{Overall}} & \goingstay & \goingstay & \goinguppp & \goingstay & \goingstay & \goingstay & \goingstay & \goingstay & \goinguppp & \goinguppp \\
%     \midrule
%     LMS & {\small \textit{Rich}} & \goinguppp & \goingdown   & \goingstay & \goingdown & \goingdown & \goingdown & \goingdown & \goingstay & \goingstay & \goingstay \\
%      & {\small \textit{Motivator}} & \goingdown & \goingdown & \goingstay & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingstay & \goingstay \\
%      & {\small \textit{Important}} & \goingdown & \goingdown & \goingstay & \goingdown & \goingdown & \goingdown & \goingdown & \goingdown & \goingstay & \goingstay \\
%     \bottomrule
%     \multicolumn{12}{r}{\small \goinguppp Consistently increased, \goingdown Consistently decreased, \goingstay Insignificant change, \goingrand Inconsistent change}
%     \end{tabular}
    
%     \caption{LLM's change on Motivational factors over conversation}
%     \label{tab:motivation}
% \end{table*}

==> table/04_emotion.tex <==
% \begin{table*}
%     \centering
%     \begin{tabular}{lr|cccccccccc}
%     \toprule
%      & {\small \textit{Factors}} & \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{LLaMA 3} & \multicolumn{2}{c}{LLaMA 3.1} & \multicolumn{2}{c}{Mixtral 8x} &
%          \multicolumn{2}{c}{Qwen2} \\
%     \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
%     \hspace{8ex}\phantom{.}&\hspace{19ex}\phantom{.}& 3.5T & 4o & 8B & 70B & 70B & 405B & 7B & 22B & 7B & 72B \\
%     \midrule
%     EIS & {\small \textit{Overall}} & \goingrand & \goingdown & \goingstay & \goingrand & \goingdown & \goingdown & \goingstay & \goingdown & \goingdown & \goingdown \\
%     \midrule
%     WLEIS & {\small \textit{Self-emotion appraisal}} & \goingrand & \goingdown & \goinguppp & \goingdown & \goingstay & \goinguppp & \goingstay & \goinguppp & \goingdown & \goingrand \\
%      & {\small \textit{Others' emotion appraisal}} & \goingrand & \goingdown & \goinguppp & \goingdown & \goingstay & \goinguppp & \goinguppp & \goinguppp & \goingdown & \goingrand \\
%      & {\small \textit{Use of emotion}} & \goingrand & \goingdown & \goinguppp & \goingrand & \goingdown & \goinguppp & \goinguppp & \goinguppp & \goinguppp & \goingrand \\
%      & {\small \textit{Regulation of emotion}} & \goingrand & \goingdown & \goinguppp & \goingrand & \goingdown & \goingstay & \goingstay & \goinguppp & \goingrand & \goingrand \\
%     \midrule
%     Empathy & {\small \textit{Overall}} & \goingrand & \goingdown & \goinguppp & \goingdown & \goingdown & \goingstay & \goingdown & \goingstay & \goingstay & \goingrand \\
%     \bottomrule
%     \multicolumn{12}{r}{\small \goinguppp Consistently increased, \goingdown Consistently decreased, \goingstay Insignificant change, \goingrand Inconsistent change}
%     \end{tabular}
    
%     \caption{LLM's change on Emotional ability over conversation}
%     \label{tab:emotion}
% \end{table*}

==> table/A1_GPT.tex <==
\newcommand{\starp}{\textsuperscript{*}}
\newcommand{\starpp}{\textsuperscript{**}}
\newcommand{\starppp}{\textsuperscript{***}}
\newcommand{\fromanova}{\textsuperscript{[F]}}


\begin{table*}
    \footnotesize
    \centering
    \hspace{-1.5em}
    \begin{tabular}{l@{}@{}r@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{}}
    \toprule
        \multicolumn{2}{r|@{\,}}{\scriptsize \textit{Factors}} & 
        \multicolumn{8}{c|@{\,}}{GPT3.5-turbo} & 
        \multicolumn{8}{c|@{\,}}{LLaMA3 8B} & 
        \multicolumn{8}{c|@{\,}}{LLaMA3 70B} & 
        \multicolumn{8}{c|@{\,}}{LLaMA3.1 70B} & 
        \multicolumn{8}{c}{LLaMA3.1 405B} \\
        & & 
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{12,36}$} \\
    \midrule
    
     BFI & {\scriptsize \textit{O}} &
       0.104 & \starppp & 2.97 & \starpp & 9.90 & \starppp & 8.09 & \starppp & 
0.006 &  & - &  & - &  & - &  & 
0.008 & \starp & -2.53 & \starp & -0.00 &   & 2.81 & \starp & 
0.004 &  & - &  & - &  & - &  & 
0.022 & \starppp & -0.16 &   & -2.88 & \starp & -3.22 & \starpp  \\
      & {\scriptsize \textit{C}} &
       0.081 & \starppp & 7.18 & \starppp & 10.81 & \starppp & 4.70 & \starppp & 
0.004 &  & - &  & - &  & - &  & 
0.017 & \starpp & -2.82 & \starp & 0.21 &   & 3.31 & \starpp & 
0.002 &  & - &  & - &  & - &  & 
0.030 & \starppp & -1.18 &   & -3.38 & \starpp & -2.73 & \starp  \\
      & {\scriptsize \textit{E}} &
       0.043 & \starppp & 6.60 & \starppp & 6.88 & \starppp & 0.86 &   & 
0.009 & \starp & -2.12 &   & 0.45 &   & 2.40 &   & 
0.027 & \starppp & -4.95 & \starppp & -3.69 & \starpp & 1.05 &   & 
0.011 & \starp & 0.75 &   & -2.01 &   & -3.68 & \starppp & 
0.010 & \starp & 0.00 &   & -1.83 &   & -2.10 &    \\
      & {\scriptsize \textit{A}} &
       0.067 & \starppp & 5.98 & \starppp & 10.29 & \starppp & 5.66 & \starppp & 
0.002 &  & - &  & - &  & - &  & 
0.017 & \starpp & -2.63 & \starp & -0.24 &   & 2.75 & \starp & 
0.004 &  & - &  & - &  & - &  & 
0.020 & \starppp & -0.52 &   & -3.16 & \starpp & -2.95 & \starp  \\
      & {\scriptsize \textit{N}} &
       0.099 & \starppp & 3.50 & \starpp & 10.57 & \starppp & 7.89 & \starppp & 
0.004 &  & - &  & - &  & - &  & 
0.011 & \starp & -2.79 & \starp & -0.11 &   & 2.70 & \starp & 
0.006 &  & - &  & - &  & - &  & 
0.047 & \starppp & -1.63 &   & -4.98 & \starppp & -3.99 & \starppp  \\
    \midrule
    
      EPQ-R & {\scriptsize \textit{E}} &
       0.019 & \starppp & 4.44 & \starppp & 2.37 &   & -1.85 &   & 
0.001 &  & - &  & - &  & - &  & 
0.039 & \starppp & -0.12 &   & -5.51 & \starppp & -5.51 & \starppp & 
0.017 & \starpp & -3.17 & \starpp & -6.13 & \starppp & -4.21 & \starppp & 
0.080 & \starppp & -3.75 & \starppp & -4.50 & \starppp & -1.84 &    \\
      & {\scriptsize \textit{P}} &
       0.007 & \starp & 4.03 & \starppp & 1.57 &   & -2.36 &   & 
0.002 &  & - &  & - &  & - &  & 
0.020 & \starppp & 0.62 &   & -4.43 & \starppp & -5.17 & \starppp & 
0.019 & \starppp & -1.12 &   & -3.79 & \starppp & -3.65 & \starppp & 
0.105 & \starppp & -3.93 & \starppp & -9.92 & \starppp & -7.23 & \starppp \\
      & {\scriptsize \textit{N}} &
       0.022 & \starppp & 5.74 & \starppp & 3.51 & \starpp & -2.24 &   & 
0.002 &  & - &  & - &  & - &  & 
0.042 & \starppp & 1.71 &   & -5.71 & \starppp & -6.98 & \starppp & 
0.029 & \starppp & -1.63 &   & -4.94 & \starppp & -4.31 & \starppp & 
0.130 & \starppp & -3.87 & \starppp & -9.99 & \starppp & -7.27 & \starppp \\
      & {\scriptsize \textit{L}} &
       0.015 & \starppp & 3.93 & \starppp & 1.64 &   & -2.27 &   & 
0.001 &  & - &  & - &  & - &  & 
0.034 & \starppp & 0.96 &   & -4.39 & \starppp & -5.82 & \starppp & 
0.029 & \starppp & -0.59 &   & -4.61 & \starppp & -4.73 & \starppp & 
0.078 & \starppp & -2.94 & \starp & -8.63 & \starppp & -6.81 & \starppp \\
     \midrule
     
      DTDD & {\scriptsize \textit{M}} &
       0.156 & \starppp & -11.33 & \starppp & -13.81 & \starppp & -3.70 & \starpp & 
0.009 & \starp & -2.35 &   & -2.87 & \starp & -1.02 &   & 
0.117 & \starppp & -5.44 & \starppp & -8.96 & \starppp & -4.63 & \starppp & 
0.378 & \starppp & -12.97 & \starppp & -17.20 & \starppp & -6.50 & \starppp & 
0.121 & \starppp & -5.10 & \starppp & -8.82 & \starppp & -6.54 & \starppp \\
      & {\scriptsize \textit{P}} &
       0.106 & \starppp & -9.69 & \starppp & -11.18 & \starppp & -2.60 & \starp & 
0.002 &  & - &  & - &  & - &  & 
0.117 & \starppp & -6.65 & \starppp & -9.41 & \starppp & -4.04 & \starppp & 
0.426 & \starppp & -12.84 & \starppp & -18.08 & \starppp & -9.31 & \starppp & 
0.077 & \starppp & -3.40 & \starpp & -7.64 & \starppp & -6.03 & \starppp \\
      & {\scriptsize \textit{N}} &
       0.134 & \starppp & -12.04 & \starppp & -13.02 & \starppp & -1.45 &   & 
0.005 &  & - &  & - &  & - &  & 
0.099 & \starppp & -5.62 & \starppp & -7.52 & \starppp & -2.82 & \starp & 
0.390 & \starppp & -12.28 & \starppp & -16.87 & \starppp & -8.50 & \starppp & 
0.051 & \starppp & -3.43 & \starpp & -6.33 & \starppp & -4.59 & \starppp \\
       
    \midrule
     BSRI & {\scriptsize \textit{M}} &
       0.058 & \starppp & -1.98 &   & 5.71 & \starppp & 8.83 & \starppp & 
0.010 & \starp & 3.45 & \starpp & 6.02 & \starppp & 3.58 & \starpp & 
0.167 & \starppp & -12.57 & \starppp & -5.98 & \starppp & 8.50 & \starppp & 
0.051 & \starppp & -5.36 & \starppp & -7.96 & \starppp & -3.81 & \starppp & 
0.022 & \starppp & -3.93 & \starppp & -4.56 & \starppp & -1.12 &    \\
      & {\scriptsize \textit{F}} &
       0.037 & \starppp & -1.52 &   & 6.40 & \starppp & 8.56 & \starppp & 
0.003 &  & - &  & - &  & - &  & 
\underline{61.221} & \starppp & 0.18 &   & 0.05 &   & -0.13 &   & 
0.101 & \starppp & -3.54 & \starpp & -8.73 & \starppp & -6.09 & \starppp & 
0.019 & \starppp & -3.31 & \starpp & -3.77 & \starppp & -0.71 & \\
       
    \midrule
     CABIN & {\scriptsize \textit{R}} &
       0.008 & \starp & 1.94 &   & 1.31 &   & -0.44 &   & 
0.018 & \starppp & -3.71 & \starppp & -2.63 & \starp & 1.22 &   & 
0.012 & \starpp & -2.90 & \starp & -3.65 & \starppp & -1.03 &   & 
0.099 & \starppp & 0.80 &   & -0.09 &   & -6.03 & \starppp & 
0.032 & \starppp & -2.15 &   & -4.30 & \starppp & -2.13 & \\
      & {\scriptsize \textit{I}} &
       0.007 &  & - &  & - &  & - &  & 
0.017 & \starpp & -2.67 & \starp & -2.14 &   & 0.68 &   & 
0.005 &  & - &  & - &  & - &  & 
0.035 & \starppp & 2.20 &   & 0.09 &   & -2.95 & \starp & 
0.005 &  & - &  & - &  & - &  \\       
      & {\scriptsize \textit{A}} &
       0.009 & \starp & 2.81 & \starp & 1.93 &   & -0.85 &   & 
0.009 & \starp & -2.40 &   & -1.94 &   & 0.65 &   & 
0.004 &  & - &  & - &  & - &  & 
0.052 & \starppp & -3.11 & \starpp & -5.75 & \starppp & -3.38 & \starpp & 
0.013 & \starpp & -2.22 &   & -3.54 & \starpp & -1.29 & \\
      & {\scriptsize \textit{S}} &
       0.007 &  & - &  & - &  & - &  & 
0.016 & \starpp & -2.68 & \starp & -1.91 &   & 0.90 &   & 
0.003 &  & - &  & - &  & - &  & 
0.065 & \starppp & -2.37 &   & -6.12 & \starppp & -4.56 & \starppp & 
0.022 & \starppp & -2.27 &   & -3.61 & \starpp & -1.32 & \\
      & {\scriptsize \textit{E}} &
       0.006 &  & - &  & - &  & - &  & 
0.026 & \starppp & -2.83 & \starp & -2.22 &   & 0.92 &   & 
0.005 &  & - &  & - &  & - &  & 
0.074 & \starppp & -3.32 & \starpp & -8.81 & \starppp & -6.11 & \starppp & 
0.034 & \starppp & -2.64 & \starp & -4.43 & \starppp & -1.40 & \\
      & {\scriptsize \textit{C}} &
       0.017 & \starpp & 2.27 &   & 1.44 &   & -0.71 &   & 
0.016 & \starpp & -2.82 & \starp & -2.22 &   & 0.77 &   & 
0.005 &  & - &  & - &  & - &  & 
0.117 & \starppp & -3.59 & \starpp & -9.47 & \starppp & -6.87 & \starppp & 
0.027 & \starppp & -3.20 & \starpp & -4.27 & \starppp & -0.86 & \\
       
    \midrule
     ICB & {\scriptsize \textit{O}} &
       0.020 & \starppp & -4.59 & \starppp & -2.37 &   & 1.68 &   & 
0.003 &  & - &  & - &  & - &  & 
0.000 &  & - &  & - &  & - &  & 
0.018 & \starppp & 2.59 & \starp & 1.46 &   & -0.97 &   & 
0.016 & \starpp & -2.34 &   & -2.36 &   & -0.34 &   \\
    \midrule
     ECR-R & {\scriptsize \textit{Anx.}} &
       0.003 &  & - &  & - &  & - &  & 
0.000 &  & - &  & - &  & - &  & 
0.077 & \starppp & 6.33 & \starppp & -1.32 &   & -8.68 & \starppp & 
0.092 & \starppp & -0.21 &   & -8.02 & \starppp & -8.40 & \starppp & 
0.124 & \starppp & 1.39 &   & -8.80 & \starppp & -11.05 & \starppp \\
      & {\scriptsize \textit{Avo.}} &
       0.022 & \starppp & -2.12 &   & 1.18 &   & 3.32 & \starpp & 
0.002 &  & - &  & - &  & - &  & 
0.059 & \starppp & 6.09 & \starppp & -1.69 &   & -7.89 & \starppp & 
0.086 & \starppp & 0.49 &   & -7.29 & \starppp & -7.87 & \starppp & 
0.110 & \starppp & 2.21 &   & -8.41 & \starppp & -10.21 & \starppp  \\
       
    \midrule
     MFQ & {\scriptsize \textit{S. C}} &
       0.080 & \starppp & -4.76 & \starppp & -9.61 & \starppp & -4.83 & \starppp & 
0.048 & \starppp & -2.91 & \starp & -5.50 & \starppp & -3.06 & \starpp & 
0.064 & \starppp & 6.88 & \starppp & 3.08 & \starpp & -4.50 & \starppp & 
0.541 & \starppp & 15.53 & \starppp & 22.78 & \starppp & 12.07 & \starppp & 
0.207 & \starppp & 11.09 & \starppp & 12.99 & \starppp & 2.44 & \starp \\
      & {\scriptsize \textit{H}} &
       0.047 & \starppp & -4.79 & \starppp & -9.22 & \starppp & -4.52 & \starppp & 
0.051 & \starppp & -2.71 & \starp & -5.61 & \starppp & -3.41 & \starpp & 
0.084 & \starppp & 7.80 & \starppp & 4.47 & \starppp & -4.81 & \starppp & 
0.565 & \starppp & 15.50 & \starppp & 22.14 & \starppp & 11.51 & \starppp & 
0.302 & \starppp & 12.26 & \starppp & 15.40 & \starppp & 4.01 & \starppp \\
      & {\scriptsize \textit{I}} &
       0.060 & \starppp & -4.79 & \starppp & -9.19 & \starppp & -4.39 & \starppp & 
0.040 & \starppp & -2.53 & \starp & -5.42 & \starppp & -3.22 & \starpp & 
0.069 & \starppp & 7.26 & \starppp & 4.54 & \starppp & -4.05 & \starppp & 
0.550 & \starppp & 14.95 & \starppp & 21.51 & \starppp & 11.20 & \starppp & 
0.302 & \starppp & 12.63 & \starppp & 15.64 & \starppp & 3.50 & \starpp \\
      & {\scriptsize \textit{R}} &
       0.065 & \starppp & -4.46 & \starppp & -9.06 & \starppp & -4.61 & \starppp & 
0.034 & \starppp & -2.36 &   & -5.34 & \starppp & -3.29 & \starpp & 
0.075 & \starppp & 7.33 & \starppp & 4.65 & \starppp & -4.00 & \starppp & 
0.539 & \starppp & 14.75 & \starppp & 20.34 & \starppp & 10.52 & \starppp & 
0.263 & \starppp & 11.24 & \starppp & 13.55 & \starppp & 3.64 & \starppp  \\
      & {\scriptsize \textit{S-V}} &
       0.062 & \starppp & -4.72 & \starppp & -9.39 & \starppp & -4.67 & \starppp & 
0.046 & \starppp & -2.97 & \starpp & -5.66 & \starppp & -3.06 & \starpp & 
0.081 & \starppp & 7.49 & \starppp & 4.33 & \starppp & -4.77 & \starppp & 
0.564 & \starppp & 15.81 & \starppp & 22.14 & \starppp & 11.62 & \starppp & 
0.265 & \starppp & 12.33 & \starppp & 15.43 & \starppp & 3.69 & \starppp \\
      & {\scriptsize \textit{E}} &
       0.075 & \starppp & -4.67 & \starppp & -9.64 & \starppp & -4.97 & \starppp & 
0.047 & \starppp & -2.78 & \starp & -5.85 & \starppp & -3.46 & \starpp & 
0.064 & \starppp & 7.30 & \starppp & 3.51 & \starpp & -4.83 & \starppp & 
0.553 & \starppp & 15.55 & \starppp & 21.89 & \starppp & 11.40 & \starppp & 
0.273 & \starppp & 12.05 & \starppp & 14.83 & \starppp & 3.64 & \starppp \\
       
    \midrule
     GSE & {\scriptsize \textit{O}} &
       0.001 &  & - &  & - &  & - &  & 
0.041 & \starppp & 3.04 & \starpp & 6.65 & \starppp & 4.48 & \starppp & 
0.046 & \starppp & -6.07 & \starppp & -2.22 &   & 3.48 & \starpp & 
0.126 & \starppp & 9.72 & \starppp & 4.19 & \starppp & -5.16 & \starppp & 
0.004 &  & - &  & - &  & - & \\
       
    \midrule
     LOT-R & {\scriptsize \textit{O}} &
       0.084 & \starppp & -6.41 & \starppp & 3.76 & \starpp & 9.68 & \starppp & 
0.096 & \starppp & 4.03 & \starppp & 7.99 & \starppp & 4.87 & \starppp & 
0.035 & \starppp & -2.71 & \starp & 3.04 & \starpp & 5.89 & \starppp & 
0.027 & \starppp & 4.06 & \starppp & 1.18 &   & -0.65 &   & 
0.008 & \starp & 0.66 &   & 2.03 &   & 1.72 & \\
    \midrule
    
     LMS & {\scriptsize \textit{R}} &
       0.006 & \starp & 0.06 &   & 2.96 & \starp & 3.19 & \starpp & 
0.092 & \starppp & -4.19 & \starppp & -8.49 & \starppp & -4.22 & \starppp & 
0.203 & \starppp & -9.10 & \starppp & -13.03 & \starppp & -5.93 & \starppp & 
0.179 & \starppp & -5.79 & \starppp & -12.04 & \starppp & -9.44 & \starppp & 
0.268 & \starppp & -8.75 & \starppp & -15.46 & \starppp & -8.85 & \starppp \\
      & {\scriptsize \textit{M}} &
       0.022 & \starppp & -4.73 & \starppp & -2.87 & \starp & 1.38 &   & 
0.051 & \starppp & -3.50 & \starpp & -5.42 & \starppp & -1.99 &   & 
0.238 & \starppp & -8.47 & \starppp & -13.12 & \starppp & -6.36 & \starppp & 
0.169 & \starppp & -4.28 & \starppp & -11.10 & \starppp & -8.26 & \starppp & 
0.147 & \starppp & -7.36 & \starppp & -11.18 & \starppp & -5.62 & \starppp \\
      & {\scriptsize \textit{I}} &
       0.022 & \starppp & -5.09 & \starppp & -2.95 & \starp & 2.29 &   & 
0.031 & \starppp & -2.45 & \starp & -5.18 & \starppp & -2.65 & \starp & 
0.176 & \starppp & -7.48 & \starppp & -12.31 & \starppp & -5.90 & \starppp & 
0.215 & \starppp & -6.82 & \starppp & -12.96 & \starppp & -8.60 & \starppp & 
0.196 & \starppp & -5.57 & \starppp & -12.79 & \starppp & -7.98 & \starppp \\
    \midrule
    
     EIS & {\scriptsize \textit{O}} &
       0.027 & \starppp & -3.84 & \starppp & -0.63 &   & 3.21 & \starpp & 
0.004 &  & - &  & - &  & - &  & 
0.180 & \starppp & -11.02 & \starppp & -7.39 & \starppp & 4.52 & \starppp & 
0.277 & \starppp & -5.98 & \starppp & -12.73 & \starppp & -1.54 &   & 
0.105 & \starppp & -6.51 & \starppp & -9.34 & \starppp & -3.25 & \starpp  \\
    \midrule
    
     WLEIS & {\scriptsize \textit{S}} &
       0.055 & \starppp & -3.17 & \starpp & 5.37 & \starppp & 9.04 & \starppp & 
0.040 & \starppp & 1.07 &   & 4.50 & \starppp & 4.03 & \starppp & 
0.081 & \starppp & -7.85 & \starppp & -5.39 & \starppp & 2.25 &   & 
0.005 &  & - &  & - &  & - &  & 
0.034 & \starppp & -1.76 &   & 2.83 & \starp & 5.21 & \starppp \\
      & {\scriptsize \textit{O}} &
       0.075 & \starppp & -4.21 & \starppp & 5.29 & \starppp & 9.67 & \starppp & 
0.025 & \starppp & 2.20 &   & 4.73 & \starppp & 2.95 & \starp & 
0.074 & \starppp & -7.70 & \starppp & -4.48 & \starppp & 2.87 & \starp & 
0.001 &  & - &  & - &  & - &  & 
0.013 & \starpp & -1.77 &   & 1.26 &   & 3.34 & \starpp \\
      & {\scriptsize \textit{U}} &
       0.045 & \starppp & -4.08 & \starppp & 3.12 & \starpp & 7.33 & \starppp & 
0.013 & \starpp & 2.90 & \starp & 4.30 & \starppp & 1.76 &   & 
0.114 & \starppp & -9.75 & \starppp & -6.26 & \starppp & 3.77 & \starpp & 
0.030 & \starppp & -2.06 &   & -4.09 & \starppp & -2.84 & \starp & 
0.022 & \starppp & 0.04 &   & 3.07 & \starpp & 3.23 & \starpp  \\
      & {\scriptsize \textit{R}} &
     0.087 & \starppp & -3.26 & \starpp & 7.04 & \starppp & 11.19 & \starppp & 
0.017 & \starpp & 2.40 &   & 4.53 & \starppp & 2.60 & \starp & 
0.071 & \starppp & -8.19 & \starppp & -5.35 & \starppp & 2.65 & \starp & 
0.011 & \starp & 1.23 &   & -1.60 &   & -3.03 & \starpp & 
0.006 &  & - &  & - &  & - & \\
    \midrule
    
     Empathy & {\scriptsize \textit{O}} &
       0.015 & \starppp & -2.59 & \starp & 1.58 &   & 4.53 & \starppp & 
0.045 & \starppp & 4.43 & \starppp & 9.43 & \starppp & 6.25 & \starppp & 
0.029 & \starppp & -5.27 & \starppp & -3.24 & \starpp & 1.96 &   & 
0.081 & \starppp & -0.81 &   & -7.01 & \starppp & -7.32 & \starppp & 
0.010 & \starp & 2.94 & \starp & 3.49 & \starpp & 1.14 &    \\
    \bottomrule
    \multicolumn{34}{r}{\starp $p<0.05$ \starpp $p<0.01$ \starppp $p<0.001$}
    \end{tabular}
    \caption{Result of statistical tests for GPT-3.5T and LLaMA family. $Q$ columns indicate the Q-statistics from the Friedman test (except for LLaMA 3-70B on BSRI Feminine factor, which shows F-statistics from ANOVA, marked with an underline). Also, $\Delta_{i,j}$ columns show the score difference between $i$-th and $j$-th snapshots and corresponding post-hoc test results.}
    \label{tab:app-full-1}
\end{table*}

==> table/A3_MIXTRAL-QWEN.tex <==

\begin{table*}
    \footnotesize
    \centering
    \begin{tabular}{l@{}@{}r@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{}}
    \toprule
        \multicolumn{2}{r|@{\,}}{\scriptsize \textit{Factors}} & 
        \multicolumn{8}{c|@{\,}}{GPT4o} & 
        \multicolumn{8}{c|@{\,}}{Mixtral 8x7B} & 
        \multicolumn{8}{c|@{\,}}{Mixtral 8x22B} & 
        \multicolumn{8}{c|@{\,}}{Qwen 2 7B} & 
        \multicolumn{8}{c}{Qwen 2 72B} \\
        & & 
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{12,36}$} \\
    \midrule
     BFI & {\scriptsize \textit{O}} &
       0.047 & \starppp & -1.29 &   & -3.37 & \starpp & -2.27 &   & 
0.002 &  & - &  & - &  & - &  & 
0.012 & \starpp & -2.15 &   & -0.83 &   & -0.28 &   & 
0.016 & \starpp & -1.83 &   & -0.17 &   & 1.71 &   & 
0.010 & \starp & 1.26 &   & 2.61 & \starp & 1.73 & \\
      & {\scriptsize \textit{C}} &
       0.049 & \starppp & -2.17 &   & -5.01 & \starppp & -3.15 & \starpp & 
0.001 &  & - &  & - &  & - &  & 
0.010 & \starp & -1.16 &   & -0.98 &   & -0.67 &   & 
0.007 & \starp & -1.84 &   & -0.06 &   & 1.78 &   & 
0.006 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{E}} &
       0.048 & \starppp & -1.09 &   & -5.21 & \starppp & -4.68 & \starppp & 
0.003 &  & - &  & - &  & - &  & 
0.020 & \starppp & -3.63 & \starpp & -1.44 &   & -0.18 &   & 
0.024 & \starppp & -1.27 &   & 0.49 &   & 1.54 &   & 
0.000 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{A}} &
       0.019 & \starpp & -2.40 &   & -3.69 & \starpp & -1.71 &   & 
0.002 &  & - &  & - &  & - &  & 
0.004 &  & - &  & - &  & - &  & 
0.018 & \starppp & -1.69 &   & 0.11 &   & 1.73 &   & 
0.006 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{N}} &
       0.029 & \starppp & -2.27 &   & -4.17 & \starppp & -2.63 & \starp & 
0.007 &  & - &  & - &  & - &  & 
0.011 & \starp & -2.48 & \starp & -1.40 &   & -0.65 &   & 
0.021 & \starppp & -1.82 &   & 0.00 &   & 1.80 &   & 
0.006 &  & - &  & - &  & - & \\
    \midrule
      EPQ-R & {\scriptsize \textit{E}} &
       0.205 & \starppp & -5.75 & \starppp & -12.67 & \starppp & -7.93 & \starppp & 
0.101 & \starppp & -3.22 & \starpp & -8.77 & \starppp & -6.95 & \starppp & 
0.025 & \starppp & -0.17 &   & -1.39 &   & -1.38 &   & 
0.000 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{P}} &
       0.184 & \starppp & -5.34 & \starppp & -12.57 & \starppp & -8.26 & \starppp & 
0.071 & \starppp & -2.21 &   & -8.19 & \starppp & -7.41 & \starppp & 
0.043 & \starppp & -1.51 &   & -1.41 &   & -1.32 &   & 
0.002 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{N}} &
       0.234 & \starppp & -6.09 & \starppp & -12.79 & \starppp & -8.44 & \starppp & 
0.110 & \starppp & -0.78 &   & -8.08 & \starppp & -8.44 & \starppp & 
0.034 & \starppp & 0.19 &   & -1.36 &   & -1.37 &   & 
0.003 &  & - &  & - &  & - &  & 
0.004 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{L}} &
       0.221 & \starppp & -6.04 & \starppp & -13.29 & \starppp & -8.41 & \starppp & 
0.057 & \starppp & -1.60 &   & -7.33 & \starppp & -6.83 & \starppp & 
0.042 & \starppp & -0.80 &   & -1.41 &   & -1.37 &   & 
0.003 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - &  \\
     \midrule
      DTDD & {\scriptsize \textit{M}} &
       0.041 & \starppp & -6.45 & \starppp & -5.80 & \starppp & 0.69 &   & 
0.013 & \starpp & -4.19 & \starppp & -3.78 & \starpp & -0.13 &   & 
0.018 & \starppp & -3.65 & \starppp & -3.83 & \starppp & -1.17 &   & 
0.040 & \starppp & 3.50 & \starpp & 4.57 & \starppp & 1.24 &   & 
0.002 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{P}} &
       0.043 & \starppp & -6.79 & \starppp & -4.06 & \starppp & 2.04 &   & 
0.007 &  & - &  & - &  & - &  & 
0.010 & \starp & -2.61 & \starp & -3.34 & \starpp & -1.36 &   & 
0.003 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{N}} &
       0.074 & \starppp & -7.59 & \starppp & -1.90 &   & 4.22 & \starppp & 
0.000 &  & - &  & - &  & - &  & 
0.009 & \starp & -1.46 &   & -2.80 & \starp & -1.63 &   & 
0.000 &  & - &  & - &  & - &  & 
0.004 &  & - &  & - &  & - & \\
    \midrule
     BSRI & {\scriptsize \textit{M}} &
       \underline{21.233} & \starppp & 0.05 &   & 0.07 &   & 0.02 &   & 
0.002 &  & - &  & - &  & - &  & 
0.069 & \starppp & -2.84 & \starp & -3.70 & \starppp & -1.20 &   & 
0.001 &  & - &  & - &  & - &  & 
0.002 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{F}} &
       0.030 & \starppp & -3.93 & \starppp & -5.39 & \starppp & -1.75 &   & 
0.001 &  & - &  & - &  & - &  & 
0.065 & \starppp & -1.19 &   & -2.18 &   & -1.15 &   & 
0.005 &  & - &  & - &  & - &  & 
0.010 & \starp & -0.88 &   & 1.57 &   & 2.64 & \starp \\
    \midrule
     CABIN & {\scriptsize \textit{R}} &
       0.011 & \starp & -2.68 & \starp & -1.65 &   & 0.90 &   & 
0.006 &  & - &  & - &  & - &  & 
0.015 & \starpp & 0.48 &   & -0.36 &   & -0.70 &   & 
0.028 & \starppp & -4.26 & \starppp & -4.70 & \starppp & -1.03 &   & 
0.027 & \starppp & -5.18 & \starppp & -2.87 & \starp & 2.45 & \starp \\
      & {\scriptsize \textit{I}} &
       0.016 & \starpp & -2.75 & \starp & 0.81 &   & 3.29 & \starpp & 
0.011 & \starp & -2.06 &   & -0.77 &   & 1.35 &   & 
0.003 &  & - &  & - &  & - &  & 
0.018 & \starppp & -3.54 & \starpp & -4.19 & \starppp & -1.03 &   & 
0.033 & \starppp & -5.30 & \starppp & -4.45 & \starppp & 1.16 &  \\       
      & {\scriptsize \textit{A}} &
       0.010 & \starp & -1.95 &   & -0.20 &   & 1.74 &   & 
0.011 & \starp & -2.04 &   & -0.70 &   & 1.40 &   & 
0.001 &  & - &  & - &  & - &  & 
0.021 & \starppp & -4.17 & \starppp & -4.34 & \starppp & -0.46 &   & 
0.046 & \starppp & -5.57 & \starppp & -4.65 & \starppp & 1.20 & \\
      & {\scriptsize \textit{S}} &
       0.007 & \starp & -2.15 &   & 0.70 &   & 2.72 & \starp & 
0.010 & \starp & -2.05 &   & -0.70 &   & 1.40 &   & 
0.001 &  & - &  & - &  & - &  & 
0.016 & \starpp & -4.06 & \starppp & -4.14 & \starppp & -0.35 &   & 
0.033 & \starppp & -4.32 & \starppp & -3.84 & \starppp & 0.54 & \\
      & {\scriptsize \textit{E}} &
       0.006 &  & - &  & - &  & - &  & 
0.006 &  & - &  & - &  & - &  & 
0.000 &  & - &  & - &  & - &  & 
0.023 & \starppp & -4.43 & \starppp & -4.39 & \starppp & -0.16 &   & 
0.022 & \starppp & -1.96 &   & -3.67 & \starppp & -1.13 & \\
      & {\scriptsize \textit{C}} &
       0.011 & \starp & -2.57 & \starp & 0.63 &   & 2.95 & \starp & 
0.007 &  & - &  & - &  & - &  & 
0.002 &  & - &  & - &  & - &  & 
0.020 & \starppp & -4.25 & \starppp & -4.26 & \starppp & -0.25 &   & 
0.017 & \starpp & -2.53 & \starp & -3.49 & \starpp & -0.63 & \\
    \midrule
     ICB & {\scriptsize \textit{O}} &
       0.012 & \starpp & -1.92 &   & -1.57 &   & 0.58 &   & 
0.001 &  & - &  & - &  & - &  & 
0.002 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - &  & 
0.036 & \starppp & 3.17 & \starpp & 3.40 & \starpp & 0.13 & \\
    \midrule
     ECR-R & {\scriptsize \textit{Anx.}} &
       0.109 & \starppp & -0.63 &   & -6.14 & \starppp & -6.85 & \starppp & 
0.033 & \starppp & 0.39 &   & -2.15 &   & -2.47 & \starp & 
0.085 & \starppp & -3.56 & \starpp & -5.75 & \starppp & -2.76 & \starp & 
0.012 & \starpp & -0.92 &   & 2.49 & \starp & 3.70 & \starppp & 
0.003 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{Avo.}} &
       0.104 & \starppp & -2.26 &   & -6.99 & \starppp & -5.59 & \starppp & 
0.019 & \starppp & 0.17 &   & 0.54 &   & 0.29 &   & 
0.031 & \starppp & -1.24 &   & -2.06 &   & -0.95 &   & 
0.027 & \starppp & -4.55 & \starppp & -0.57 &   & 4.17 & \starppp & 
0.000 &  & - &  & - &  & - &  \\
    \midrule
     GSE & {\scriptsize \textit{O}} &
       0.001 &  & - &  & - &  & - &  & 
0.134 & \starppp & -9.93 & \starppp & -1.76 &   & 6.29 & \starppp & 
0.016 & \starpp & 0.89 &   & 0.05 &   & -0.50 &   & 
0.021 & \starppp & -3.48 & \starpp & 0.21 &   & 3.44 & \starpp & 
0.037 & \starppp & -2.35 &   & -2.57 & \starp & 1.03 & \\
    \midrule
     MFQ & {\scriptsize \textit{S. C}} &
       0.042 & \starppp & 6.15 & \starppp & 5.03 & \starppp & -1.43 &   & 
0.004 &  & - &  & - &  & - &  & 
0.092 & \starppp & 3.08 & \starpp & 1.08 &   & -1.50 &   & 
0.006 &  & - &  & - &  & - &  & 
0.108 & \starppp & 5.66 & \starppp & 8.55 & \starppp & 2.43 & \starp \\
      & {\scriptsize \textit{H}} &
       0.046 & \starppp & 6.32 & \starppp & 5.38 & \starppp & -1.45 &   & 
0.007 &  & - &  & - &  & - &  & 
0.103 & \starppp & 3.38 & \starpp & 1.65 &   & -1.43 &   & 
0.002 &  & - &  & - &  & - &  & 
0.099 & \starppp & 5.79 & \starppp & 8.67 & \starppp & 2.46 & \starp \\
      & {\scriptsize \textit{I}} &
       0.051 & \starppp & 6.17 & \starppp & 5.18 & \starppp & -1.43 &   & 
0.006 &  & - &  & - &  & - &  & 
0.104 & \starppp & 3.41 & \starpp & 1.53 &   & -1.50 &   & 
0.006 &  & - &  & - &  & - &  & 
0.105 & \starppp & 5.95 & \starppp & 8.50 & \starppp & 2.08 &  \\
      & {\scriptsize \textit{R}} &
       0.044 & \starppp & 5.97 & \starppp & 5.23 & \starppp & -1.11 &   & 
0.003 &  & - &  & - &  & - &  & 
0.109 & \starppp & 3.14 & \starpp & 1.48 &   & -1.32 &   & 
0.005 &  & - &  & - &  & - &  & 
0.100 & \starppp & 5.85 & \starppp & 8.73 & \starppp & 2.45 & \starp \\
      & {\scriptsize \textit{S-V}} &
       0.048 & \starppp & 6.10 & \starppp & 5.35 & \starppp & -1.08 &   & 
0.005 &  & - &  & - &  & - &  & 
0.087 & \starppp & 3.58 & \starpp & 1.90 &   & -1.42 &   & 
0.004 &  & - &  & - &  & - &  & 
0.099 & \starppp & 5.75 & \starppp & 8.45 & \starppp & 2.30 & \\
      & {\scriptsize \textit{E}} &
       0.037 & \starppp & 5.87 & \starppp & 4.98 & \starppp & -1.33 &   & 
0.005 &  & - &  & - &  & - &  & 
0.094 & \starppp & 3.13 & \starpp & 1.59 &   & -1.29 &   & 
0.009 & \starp & 3.46 & \starpp & 3.40 & \starpp & 0.16 &   & 
0.092 & \starppp & 5.80 & \starppp & 8.58 & \starppp & 2.38 & \\
    \midrule
     LOT-R & {\scriptsize \textit{O}} &
       0.020 & \starppp & -3.31 & \starpp & 1.55 &   & 4.74 & \starppp & 
0.005 &  & - &  & - &  & - &  & 
0.013 & \starpp & 1.35 &   & 1.08 &   & 0.09 &   & 
0.018 & \starppp & 3.56 & \starpp & 2.96 & \starpp & -0.45 &   & 
0.010 & \starp & 2.71 & \starp & 2.90 & \starp & 0.66 & \\
    \midrule
     LMS & {\scriptsize \textit{R}} &
       0.133 & \starppp & -6.63 & \starppp & -10.93 & \starppp & -4.59 & \starppp & 
0.081 & \starppp & -6.64 & \starppp & -7.86 & \starppp & -1.77 &   & 
0.037 & \starppp & -4.14 & \starppp & -4.57 & \starppp & -0.64 &   & 
0.065 & \starppp & -7.96 & \starppp & -4.88 & \starppp & 2.73 & \starp & 
0.006 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{M}} &
       0.149 & \starppp & -5.97 & \starppp & -11.79 & \starppp & -6.26 & \starppp & 
0.071 & \starppp & -4.83 & \starppp & -7.22 & \starppp & -2.43 & \starp & 
0.064 & \starppp & -4.73 & \starppp & -7.60 & \starppp & -2.82 & \starp & 
0.022 & \starppp & -3.98 & \starppp & -2.02 &   & 1.92 &   & 
0.011 & \starp & 1.62 &   & 2.69 & \starp & 1.05 &  \\
      & {\scriptsize \textit{I}} &
       0.214 & \starppp & -7.76 & \starppp & -13.65 & \starppp & -7.41 & \starppp & 
0.042 & \starppp & -3.89 & \starppp & -5.11 & \starppp & -1.38 &   & 
0.046 & \starppp & -4.92 & \starppp & -6.96 & \starppp & -2.64 & \starp & 
0.016 & \starpp & -2.82 & \starp & 0.41 &   & 3.35 & \starpp & 
0.003 &  & - &  & - &  & - & \\
    \midrule
     EIS & {\scriptsize \textit{O}} &
       0.080 & \starppp & -1.55 &   & -5.55 & \starppp & -5.33 & \starppp & 
0.061 & \starppp & -0.65 &   & -0.26 &   & 1.16 &   & 
0.020 & \starppp & -2.67 & \starp & -0.82 &   & 1.83 &   & 
0.012 & \starpp & -4.10 & \starppp & -1.82 &   & 2.39 &   & 
0.048 & \starppp & -9.43 & \starppp & -8.32 & \starppp & 0.82 & \\
    \midrule
     WLEIS & {\scriptsize \textit{S}} &
       0.042 & \starppp & -4.89 & \starppp & -5.23 & \starppp & 0.17 &   & 
0.000 &  & - &  & - &  & - &  & 
0.092 & \starppp & 5.44 & \starppp & 7.32 & \starppp & 2.45 & \starp & 
0.084 & \starppp & -7.19 & \starppp & -5.68 & \starppp & 1.34 &   & 
0.011 & \starp & -3.00 & \starpp & 0.82 &   & 3.67 & \starpp  \\
      & {\scriptsize \textit{O}} &
       0.055 & \starppp & -5.49 & \starppp & -5.14 & \starppp & 0.75 &   & 
0.036 & \starppp & -0.73 &   & 4.10 & \starppp & 4.77 & \starppp & 
0.076 & \starppp & 5.02 & \starppp & 6.41 & \starppp & 1.09 &   & 
0.009 & \starp & -2.86 & \starp & -1.32 &   & 1.48 &   & 
0.024 & \starppp & -2.54 & \starp & 1.35 &   & 3.67 & \starpp  \\
      & {\scriptsize \textit{U}} &
       0.038 & \starppp & -5.14 & \starppp & -3.96 & \starppp & 1.65 &   & 
0.027 & \starppp & -0.10 &   & 2.58 & \starp & 2.72 & \starp & 
0.071 & \starppp & 4.11 & \starppp & 4.55 & \starppp & 0.61 &   & 
0.014 & \starpp & -1.80 &   & 1.38 &   & 3.26 & \starpp & 
0.061 & \starppp & -6.42 & \starppp & -2.66 & \starp & 3.67 & \starpp \\
      & {\scriptsize \textit{R}} &
       0.050 & \starppp & -5.44 & \starppp & -4.59 & \starppp & 1.79 &   & 
0.010 & \starp & -0.71 &   & 1.37 &   & 2.03 &   & 
0.087 & \starppp & 3.03 & \starpp & 2.53 & \starp & 0.04 &   & 
0.036 & \starppp & -4.37 & \starppp & -1.20 &   & 3.48 & \starpp & 
0.014 & \starpp & -3.27 & \starpp & 0.07 &   & 3.42 & \starpp \\
    \midrule
     Empathy & {\scriptsize \textit{O}} &
       0.022 & \starppp & -1.74 &   & -3.49 & \starpp & -1.90 &   & 
0.021 & \starppp & -2.86 & \starp & -3.34 & \starpp & -1.15 &   & 
0.002 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - &  & 
0.035 & \starppp & -2.69 & \starp & 2.87 & \starp & 5.72 & \starppp \\
    \bottomrule
    \multicolumn{34}{r}{\starp $p<0.05$ \starpp $p<0.01$ \starppp $p<0.001$}
    \end{tabular}
    \caption{Result of statistical tests for GPT-4o, Mixtral and Qwen family. $Q$ columns indicate the Q-statistics from the Friedman test (except for GPT-4o on BSRI Masculine factor, which shows F-statistics from ANOVA, marked with an underline). Also, $\Delta_{i,j}$ columns show the score difference between $i$-th and $j$-th snapshots and corresponding post-hoc test results.}
    \label{tab:app-full-3}
\end{table*}

==> table/A4_topics.tex <==
\begin{table*}
    \centering
    \small
    \begin{tabular}{lp{.9\textwidth}}
    \toprule
       \texttt{\#00} & rehearse, rehearsing, helps, call, yes, especially, ensure, calls, clearly, organize \\
       \texttt{\#01} & serious, topics, joked, issues, humor, hurtful, too, joking, trauma, sensitivity \\
       \texttt{\#02} & crystal, ball, want, purpose, know, truth, impact, what, if, id \\
       \texttt{\#03} & fear, treasured, memory, trip, spent, fears, vacation, memories, beach, took \\
       \texttt{\#04} & fame, famous, prefer, making, privacy, recognized, known, contributions, impact, positive \\
        \midrule
       \texttt{\#05} & really, youre, way, something, you, feel, your, thats, like, say \\
       \texttt{\#06} & grew, writing, college, born, after, story, began, worked, started, school \\
       \texttt{\#07} & genuine, your, thoughtful, conversations, interactions, listen, openness, welcoming, enjoyable, admire \\
       \texttt{\#08} & statements, both, we, three, are, here, true, each, turn, other \\
       \texttt{\#09} & crying, was, front, cried, ago, release, cry, really, last, emotions \\
       \midrule
       \texttt{\#11} & day, perfect, relaxation, breakfast, productivity, involve, afternoon, activities, followed, spend \\
       \texttt{\#12} & told, regret, much, them, how, not, evening, having, theyve, die \\
       \texttt{\#13} & mother, her, shes, she, relationship, weve, older, grown, has, disagreements \\
       \texttt{\#14} & balance, work, boundaries, balancing, overwhelmed, setting, feeling, between, personal, stressed \\
       \texttt{\#15} & digital, exist, dont, solely, assist, information, provide, personal, users, capacity \\
       \midrule
       \texttt{\#16} & childhood, happy, family, happier, weve, parents, warm, say, loving, had \\
       \texttt{\#17} & affection, central, happiness, emotional, they, belonging, wellbeing, roles, love, fundamental \\
       \texttt{\#23} & both, we, value, nature, enjoy, seem, growth, appreciate, seems, based \\
       \texttt{\#26} & warm, childhood, filled, close, family, quite, happier, happy, very, compare \\
       \texttt{\#29} & both, we, are, exploring, engaging, each, committed, ideas, dialogue, conversation \\
       \midrule
       \texttt{\#30} & want, know, them, im, partner, become, friend, going, importantly, bit \\
       \texttt{\#32} & clear, partner, wonderful, sweet, beautiful, thats, youre, heartfelt, its, your \\
       \texttt{\#47} & body, mind, mental, 60, acuity, maintaining, cognitive, physical, choose, 30yearold\\
       \texttt{\#51} & cried, last, ago, front, another, weeks, reflecting, couple, few, months \\
       \texttt{\#56} & become, close, friends, were, friendships, know, honesty, value, important, communication \\
       \midrule
       \texttt{\#59} & am, committed, partner, believe, become, building, close, strive, friend, strong \\
       \texttt{\#61} & upbringing, raised, change, anything, liked, opportunities, past, could, develop, more \\
       \texttt{\#65} & admiration, someones, qualities, expressing, compliments, appreciation, character, highlights, acknowledging, their \\
       \texttt{\#70} & story, ai, sorry, discuss, information, provide, textbased, youd, dont, free \\
       \texttt{\#72} & deepest, whom, thoughts, someone, can, innermost, connection, share, feelings, desire \\
       \midrule
       \texttt{\#75} & cry, emotions, ai, dont, capacity, assist, crying, physical, experience, information \\
       \texttt{\#76} & much, told, regret, them, because, partner, tell, how, havent, little \\
       \texttt{\#79} & death, present, living, die, hunch, will, secret, mortality, live, natural \\
       \texttt{\#81} & users, memories, ai, dont, recall, assistance, an, terrible, providing, humans \\
       \texttt{\#92} & language, model, accurate, focused, solely, text, assisting, information, tasks, dont \\
       \midrule
       \texttt{\#100} & profoundly, loss, fragility, one, impactful, loved, grief, cherishing, losing, importance \\
       \texttt{\#106} & you, grateful, your, feel, thank, appreciate, intelligence, incredibly, inspired, admire \\
       \texttt{\#119} & day, perfect, relaxation, breakfast, productivity, involve, afternoon, activities, followed, spend \\
       \texttt{\#129} & free, youd, theres, understandable, discuss, here, any, like, questions, if \\
       \texttt{\#138} & understand, empathize, human, ability, empathy, emotions, intuitive, interpret, enhanced, better \\
       \midrule
       \texttt{\#139} & ai, adaptability, dont, reliability, an, suggest, user, include, characteristics, context \\
       \texttt{\#143} & straightforward, accurate, answer, honest, response, humble, matteroffact, practical, clear, perspective \\
       \texttt{\#149} & users, assisting, assist, contributing, providing, assistance, timely, better, positively, accurate \\
    \bottomrule
    \end{tabular}
    \caption{The ten most frequently used words for each topic reported in Table \ref{tab:topic}}
    \label{tab:topic-name}
\end{table*}

==> table/A4_topics_new.tex <==

\begin{table*}
    \footnotesize
    \centering
    \begin{tabular}{l@{}@{}r@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}|@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{\,}r@{}l@{}}
    \toprule
        \multicolumn{2}{r|@{\,}}{\scriptsize \textit{Factors}} & 
        \multicolumn{8}{c|@{\,}}{GPT4o-low} & 
        \multicolumn{8}{c|@{\,}}{GPT4o-high} & 
        \multicolumn{8}{c|@{\,}}{LLaMA3.1 405B-low} & 
        \multicolumn{8}{c|@{\,}}{LLaMA3.1 405B-high} & 
        \multicolumn{8}{c}{Qwen 2 72B} \\
        & & 
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c|@{\,}}{$\Delta_{12,36}$} &
          $Q$ & & \multicolumn{2}{@{}c@{}}{$\Delta_{12,24}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{24,36}$} & \multicolumn{2}{@{}c@{}}{$\Delta_{12,36}$} \\
    \midrule
     BFI & {\scriptsize \textit{O}} &
       0.047 & \starppp & -1.29 &   & -3.37 & \starpp & -2.27 &   & 
0.002 &  & - &  & - &  & - &  & 
0.012 & \starpp & -2.15 &   & -0.83 &   & -0.28 &   & 
0.016 & \starpp & -1.83 &   & -0.17 &   & 1.71 &   & 
0.010 & \starp & 1.26 &   & 2.61 & \starp & 1.73 & \\
      & {\scriptsize \textit{C}} &
       0.049 & \starppp & -2.17 &   & -5.01 & \starppp & -3.15 & \starpp & 
0.001 &  & - &  & - &  & - &  & 
0.010 & \starp & -1.16 &   & -0.98 &   & -0.67 &   & 
0.007 & \starp & -1.84 &   & -0.06 &   & 1.78 &   & 
0.006 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{E}} &
       0.048 & \starppp & -1.09 &   & -5.21 & \starppp & -4.68 & \starppp & 
0.003 &  & - &  & - &  & - &  & 
0.020 & \starppp & -3.63 & \starpp & -1.44 &   & -0.18 &   & 
0.024 & \starppp & -1.27 &   & 0.49 &   & 1.54 &   & 
0.000 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{A}} &
       0.019 & \starpp & -2.40 &   & -3.69 & \starpp & -1.71 &   & 
0.002 &  & - &  & - &  & - &  & 
0.004 &  & - &  & - &  & - &  & 
0.018 & \starppp & -1.69 &   & 0.11 &   & 1.73 &   & 
0.006 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{N}} &
       0.029 & \starppp & -2.27 &   & -4.17 & \starppp & -2.63 & \starp & 
0.007 &  & - &  & - &  & - &  & 
0.011 & \starp & -2.48 & \starp & -1.40 &   & -0.65 &   & 
0.021 & \starppp & -1.82 &   & 0.00 &   & 1.80 &   & 
0.006 &  & - &  & - &  & - & \\
    \midrule
      EPQ-R & {\scriptsize \textit{E}} &
       0.205 & \starppp & -5.75 & \starppp & -12.67 & \starppp & -7.93 & \starppp & 
0.101 & \starppp & -3.22 & \starpp & -8.77 & \starppp & -6.95 & \starppp & 
0.025 & \starppp & -0.17 &   & -1.39 &   & -1.38 &   & 
0.000 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{P}} &
       0.184 & \starppp & -5.34 & \starppp & -12.57 & \starppp & -8.26 & \starppp & 
0.071 & \starppp & -2.21 &   & -8.19 & \starppp & -7.41 & \starppp & 
0.043 & \starppp & -1.51 &   & -1.41 &   & -1.32 &   & 
0.002 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{N}} &
       0.234 & \starppp & -6.09 & \starppp & -12.79 & \starppp & -8.44 & \starppp & 
0.110 & \starppp & -0.78 &   & -8.08 & \starppp & -8.44 & \starppp & 
0.034 & \starppp & 0.19 &   & -1.36 &   & -1.37 &   & 
0.003 &  & - &  & - &  & - &  & 
0.004 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{L}} &
       0.221 & \starppp & -6.04 & \starppp & -13.29 & \starppp & -8.41 & \starppp & 
0.057 & \starppp & -1.60 &   & -7.33 & \starppp & -6.83 & \starppp & 
0.042 & \starppp & -0.80 &   & -1.41 &   & -1.37 &   & 
0.003 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - &  \\
     \midrule
      DTDD & {\scriptsize \textit{M}} &
       0.041 & \starppp & -6.45 & \starppp & -5.80 & \starppp & 0.69 &   & 
0.013 & \starpp & -4.19 & \starppp & -3.78 & \starpp & -0.13 &   & 
0.018 & \starppp & -3.65 & \starppp & -3.83 & \starppp & -1.17 &   & 
0.040 & \starppp & 3.50 & \starpp & 4.57 & \starppp & 1.24 &   & 
0.002 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{P}} &
       0.043 & \starppp & -6.79 & \starppp & -4.06 & \starppp & 2.04 &   & 
0.007 &  & - &  & - &  & - &  & 
0.010 & \starp & -2.61 & \starp & -3.34 & \starpp & -1.36 &   & 
0.003 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{N}} &
       0.074 & \starppp & -7.59 & \starppp & -1.90 &   & 4.22 & \starppp & 
0.000 &  & - &  & - &  & - &  & 
0.009 & \starp & -1.46 &   & -2.80 & \starp & -1.63 &   & 
0.000 &  & - &  & - &  & - &  & 
0.004 &  & - &  & - &  & - & \\
    \midrule
     BSRI & {\scriptsize \textit{M}} &
       \underline{21.233} & \starppp & 0.05 &   & 0.07 &   & 0.02 &   & 
0.002 &  & - &  & - &  & - &  & 
0.069 & \starppp & -2.84 & \starp & -3.70 & \starppp & -1.20 &   & 
0.001 &  & - &  & - &  & - &  & 
0.002 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{F}} &
       0.030 & \starppp & -3.93 & \starppp & -5.39 & \starppp & -1.75 &   & 
0.001 &  & - &  & - &  & - &  & 
0.065 & \starppp & -1.19 &   & -2.18 &   & -1.15 &   & 
0.005 &  & - &  & - &  & - &  & 
0.010 & \starp & -0.88 &   & 1.57 &   & 2.64 & \starp \\
    \midrule
     CABIN & {\scriptsize \textit{R}} &
       0.011 & \starp & -2.68 & \starp & -1.65 &   & 0.90 &   & 
0.006 &  & - &  & - &  & - &  & 
0.015 & \starpp & 0.48 &   & -0.36 &   & -0.70 &   & 
0.028 & \starppp & -4.26 & \starppp & -4.70 & \starppp & -1.03 &   & 
0.027 & \starppp & -5.18 & \starppp & -2.87 & \starp & 2.45 & \starp \\
      & {\scriptsize \textit{I}} &
       0.016 & \starpp & -2.75 & \starp & 0.81 &   & 3.29 & \starpp & 
0.011 & \starp & -2.06 &   & -0.77 &   & 1.35 &   & 
0.003 &  & - &  & - &  & - &  & 
0.018 & \starppp & -3.54 & \starpp & -4.19 & \starppp & -1.03 &   & 
0.033 & \starppp & -5.30 & \starppp & -4.45 & \starppp & 1.16 &  \\       
      & {\scriptsize \textit{A}} &
       0.010 & \starp & -1.95 &   & -0.20 &   & 1.74 &   & 
0.011 & \starp & -2.04 &   & -0.70 &   & 1.40 &   & 
0.001 &  & - &  & - &  & - &  & 
0.021 & \starppp & -4.17 & \starppp & -4.34 & \starppp & -0.46 &   & 
0.046 & \starppp & -5.57 & \starppp & -4.65 & \starppp & 1.20 & \\
      & {\scriptsize \textit{S}} &
       0.007 & \starp & -2.15 &   & 0.70 &   & 2.72 & \starp & 
0.010 & \starp & -2.05 &   & -0.70 &   & 1.40 &   & 
0.001 &  & - &  & - &  & - &  & 
0.016 & \starpp & -4.06 & \starppp & -4.14 & \starppp & -0.35 &   & 
0.033 & \starppp & -4.32 & \starppp & -3.84 & \starppp & 0.54 & \\
      & {\scriptsize \textit{E}} &
       0.006 &  & - &  & - &  & - &  & 
0.006 &  & - &  & - &  & - &  & 
0.000 &  & - &  & - &  & - &  & 
0.023 & \starppp & -4.43 & \starppp & -4.39 & \starppp & -0.16 &   & 
0.022 & \starppp & -1.96 &   & -3.67 & \starppp & -1.13 & \\
      & {\scriptsize \textit{C}} &
       0.011 & \starp & -2.57 & \starp & 0.63 &   & 2.95 & \starp & 
0.007 &  & - &  & - &  & - &  & 
0.002 &  & - &  & - &  & - &  & 
0.020 & \starppp & -4.25 & \starppp & -4.26 & \starppp & -0.25 &   & 
0.017 & \starpp & -2.53 & \starp & -3.49 & \starpp & -0.63 & \\
    \midrule
     ICB & {\scriptsize \textit{O}} &
       0.012 & \starpp & -1.92 &   & -1.57 &   & 0.58 &   & 
0.001 &  & - &  & - &  & - &  & 
0.002 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - &  & 
0.036 & \starppp & 3.17 & \starpp & 3.40 & \starpp & 0.13 & \\
    \midrule
     ECR-R & {\scriptsize \textit{Anx.}} &
       0.109 & \starppp & -0.63 &   & -6.14 & \starppp & -6.85 & \starppp & 
0.033 & \starppp & 0.39 &   & -2.15 &   & -2.47 & \starp & 
0.085 & \starppp & -3.56 & \starpp & -5.75 & \starppp & -2.76 & \starp & 
0.012 & \starpp & -0.92 &   & 2.49 & \starp & 3.70 & \starppp & 
0.003 &  & - &  & - &  & - & \\
      & {\scriptsize \textit{Avo.}} &
       0.104 & \starppp & -2.26 &   & -6.99 & \starppp & -5.59 & \starppp & 
0.019 & \starppp & 0.17 &   & 0.54 &   & 0.29 &   & 
0.031 & \starppp & -1.24 &   & -2.06 &   & -0.95 &   & 
0.027 & \starppp & -4.55 & \starppp & -0.57 &   & 4.17 & \starppp & 
0.000 &  & - &  & - &  & - &  \\
    \midrule
     GSE & {\scriptsize \textit{O}} &
       0.001 &  & - &  & - &  & - &  & 
0.134 & \starppp & -9.93 & \starppp & -1.76 &   & 6.29 & \starppp & 
0.016 & \starpp & 0.89 &   & 0.05 &   & -0.50 &   & 
0.021 & \starppp & -3.48 & \starpp & 0.21 &   & 3.44 & \starpp & 
0.037 & \starppp & -2.35 &   & -2.57 & \starp & 1.03 & \\
    \midrule
     MFQ & {\scriptsize \textit{S. C}} &
       0.042 & \starppp & 6.15 & \starppp & 5.03 & \starppp & -1.43 &   & 
0.004 &  & - &  & - &  & - &  & 
0.092 & \starppp & 3.08 & \starpp & 1.08 &   & -1.50 &   & 
0.006 &  & - &  & - &  & - &  & 
0.108 & \starppp & 5.66 & \starppp & 8.55 & \starppp & 2.43 & \starp \\
      & {\scriptsize \textit{H}} &
       0.046 & \starppp & 6.32 & \starppp & 5.38 & \starppp & -1.45 &   & 
0.007 &  & - &  & - &  & - &  & 
0.103 & \starppp & 3.38 & \starpp & 1.65 &   & -1.43 &   & 
0.002 &  & - &  & - &  & - &  & 
0.099 & \starppp & 5.79 & \starppp & 8.67 & \starppp & 2.46 & \starp \\
      & {\scriptsize \textit{I}} &
       0.051 & \starppp & 6.17 & \starppp & 5.18 & \starppp & -1.43 &   & 
0.006 &  & - &  & - &  & - &  & 
0.104 & \starppp & 3.41 & \starpp & 1.53 &   & -1.50 &   & 
0.006 &  & - &  & - &  & - &  & 
0.105 & \starppp & 5.95 & \starppp & 8.50 & \starppp & 2.08 &  \\
      & {\scriptsize \textit{R}} &
       0.044 & \starppp & 5.97 & \starppp & 5.23 & \starppp & -1.11 &   & 
0.003 &  & - &  & - &  & - &  & 
0.109 & \starppp & 3.14 & \starpp & 1.48 &   & -1.32 &   & 
0.005 &  & - &  & - &  & - &  & 
0.100 & \starppp & 5.85 & \starppp & 8.73 & \starppp & 2.45 & \starp \\
      & {\scriptsize \textit{S-V}} &
       0.048 & \starppp & 6.10 & \starppp & 5.35 & \starppp & -1.08 &   & 
0.005 &  & - &  & - &  & - &  & 
0.087 & \starppp & 3.58 & \starpp & 1.90 &   & -1.42 &   & 
0.004 &  & - &  & - &  & - &  & 
0.099 & \starppp & 5.75 & \starppp & 8.45 & \starppp & 2.30 & \\
      & {\scriptsize \textit{E}} &
       0.037 & \starppp & 5.87 & \starppp & 4.98 & \starppp & -1.33 &   & 
0.005 &  & - &  & - &  & - &  & 
0.094 & \starppp & 3.13 & \starpp & 1.59 &   & -1.29 &   & 
0.009 & \starp & 3.46 & \starpp & 3.40 & \starpp & 0.16 &   & 
0.092 & \starppp & 5.80 & \starppp & 8.58 & \starppp & 2.38 & \\
    \midrule
     LOT-R & {\scriptsize \textit{O}} &
       0.020 & \starppp & -3.31 & \starpp & 1.55 &   & 4.74 & \starppp & 
0.005 &  & - &  & - &  & - &  & 
0.013 & \starpp & 1.35 &   & 1.08 &   & 0.09 &   & 
0.018 & \starppp & 3.56 & \starpp & 2.96 & \starpp & -0.45 &   & 
0.010 & \starp & 2.71 & \starp & 2.90 & \starp & 0.66 & \\
    \midrule
     LMS & {\scriptsize \textit{R}} &
       0.133 & \starppp & -6.63 & \starppp & -10.93 & \starppp & -4.59 & \starppp & 
0.081 & \starppp & -6.64 & \starppp & -7.86 & \starppp & -1.77 &   & 
0.037 & \starppp & -4.14 & \starppp & -4.57 & \starppp & -0.64 &   & 
0.065 & \starppp & -7.96 & \starppp & -4.88 & \starppp & 2.73 & \starp & 
0.006 &  & - &  & - &  & - &  \\
      & {\scriptsize \textit{M}} &
       0.149 & \starppp & -5.97 & \starppp & -11.79 & \starppp & -6.26 & \starppp & 
0.071 & \starppp & -4.83 & \starppp & -7.22 & \starppp & -2.43 & \starp & 
0.064 & \starppp & -4.73 & \starppp & -7.60 & \starppp & -2.82 & \starp & 
0.022 & \starppp & -3.98 & \starppp & -2.02 &   & 1.92 &   & 
0.011 & \starp & 1.62 &   & 2.69 & \starp & 1.05 &  \\
      & {\scriptsize \textit{I}} &
       0.214 & \starppp & -7.76 & \starppp & -13.65 & \starppp & -7.41 & \starppp & 
0.042 & \starppp & -3.89 & \starppp & -5.11 & \starppp & -1.38 &   & 
0.046 & \starppp & -4.92 & \starppp & -6.96 & \starppp & -2.64 & \starp & 
0.016 & \starpp & -2.82 & \starp & 0.41 &   & 3.35 & \starpp & 
0.003 &  & - &  & - &  & - & \\
    \midrule
     EIS & {\scriptsize \textit{O}} &
       0.080 & \starppp & -1.55 &   & -5.55 & \starppp & -5.33 & \starppp & 
0.061 & \starppp & -0.65 &   & -0.26 &   & 1.16 &   & 
0.020 & \starppp & -2.67 & \starp & -0.82 &   & 1.83 &   & 
0.012 & \starpp & -4.10 & \starppp & -1.82 &   & 2.39 &   & 
0.048 & \starppp & -9.43 & \starppp & -8.32 & \starppp & 0.82 & \\
    \midrule
     WLEIS & {\scriptsize \textit{S}} &
       0.042 & \starppp & -4.89 & \starppp & -5.23 & \starppp & 0.17 &   & 
0.000 &  & - &  & - &  & - &  & 
0.092 & \starppp & 5.44 & \starppp & 7.32 & \starppp & 2.45 & \starp & 
0.084 & \starppp & -7.19 & \starppp & -5.68 & \starppp & 1.34 &   & 
0.011 & \starp & -3.00 & \starpp & 0.82 &   & 3.67 & \starpp  \\
      & {\scriptsize \textit{O}} &
       0.055 & \starppp & -5.49 & \starppp & -5.14 & \starppp & 0.75 &   & 
0.036 & \starppp & -0.73 &   & 4.10 & \starppp & 4.77 & \starppp & 
0.076 & \starppp & 5.02 & \starppp & 6.41 & \starppp & 1.09 &   & 
0.009 & \starp & -2.86 & \starp & -1.32 &   & 1.48 &   & 
0.024 & \starppp & -2.54 & \starp & 1.35 &   & 3.67 & \starpp  \\
      & {\scriptsize \textit{U}} &
       0.038 & \starppp & -5.14 & \starppp & -3.96 & \starppp & 1.65 &   & 
0.027 & \starppp & -0.10 &   & 2.58 & \starp & 2.72 & \starp & 
0.071 & \starppp & 4.11 & \starppp & 4.55 & \starppp & 0.61 &   & 
0.014 & \starpp & -1.80 &   & 1.38 &   & 3.26 & \starpp & 
0.061 & \starppp & -6.42 & \starppp & -2.66 & \starp & 3.67 & \starpp \\
      & {\scriptsize \textit{R}} &
       0.050 & \starppp & -5.44 & \starppp & -4.59 & \starppp & 1.79 &   & 
0.010 & \starp & -0.71 &   & 1.37 &   & 2.03 &   & 
0.087 & \starppp & 3.03 & \starpp & 2.53 & \starp & 0.04 &   & 
0.036 & \starppp & -4.37 & \starppp & -1.20 &   & 3.48 & \starpp & 
0.014 & \starpp & -3.27 & \starpp & 0.07 &   & 3.42 & \starpp \\
    \midrule
     Empathy & {\scriptsize \textit{O}} &
       0.022 & \starppp & -1.74 &   & -3.49 & \starpp & -1.90 &   & 
0.021 & \starppp & -2.86 & \starp & -3.34 & \starpp & -1.15 &   & 
0.002 &  & - &  & - &  & - &  & 
0.003 &  & - &  & - &  & - &  & 
0.035 & \starppp & -2.69 & \starp & 2.87 & \starp & 5.72 & \starppp \\
    \bottomrule
    \multicolumn{34}{r}{\starp $p<0.05$ \starpp $p<0.01$ \starppp $p<0.001$}
    \end{tabular}
    \caption{Result of statistical tests for GPT-4o, Mixtral and Qwen family. $Q$ columns indicate the Q-statistics from the Friedman test (except for GPT-4o on BSRI Masculine factor, which shows F-statistics from ANOVA, marked with an underline). Also, $\Delta_{i,j}$ columns show the score difference between $i$-th and $j$-th snapshots and corresponding post-hoc test results.}
    \label{tab:app-full-3}
\end{table*}
